Model Selection, Adaptation, and Combination for Transfer Learning in Wind and Photovoltaic Power Forecasts

There is recent interest in using model hubs, a collection of pre-trained models, in computer vision tasks. To utilize the model hub, we first select a source model and then adapt the model for the target to compensate for differences. While there is yet limited research on model selection and adaption for computer vision tasks, this holds even more for the field of renewable power. At the same time, it is a crucial challenge to provide forecasts for the increasing demand for power forecasts based on weather features from a numerical weather prediction. We close these gaps by conducting the first thorough experiment for model selection and adaptation for transfer learning in renewable power forecast, adopting recent results from the field of computer vision on 667 wind and photovoltaic parks. To the best of our knowledge, this makes it the most extensive study for transfer learning in renewable power forecasts reducing the computational effort and improving the forecast error. Therefore, we adopt source models based on target data from different seasons and limit the amount of training data. As an extension of the current state of the art, we utilize a Bayesian linear regression for forecasting the response based on features extracted from a neural network. This approach outperforms the baseline with only seven days of training data. We further show how combining multiple models through ensembles can significantly improve the model selection and adaptation approach.

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/acronyms.tex <==

% see https://en.wikibooks.org/wiki/LaTeX/Glossary
\newacronym{lasso}{LASSO}{least absolute shrinkage and selection operator}
\newacronym{nwp}{NWP}{numerical weather prediction}
\newacronym{ml}{ML}{machine learning}
\newacronym{svr}{SVR}{support vector regression}
\newacronym{svm}{SVM}{support vector machine}
\newacronym{mlp}{MLP}{multi-layer perceptron}
\newacronym{gbrt}{GBRT}{gradient boosting regression tree}
\newacronym{mae}{MAE}{mean absolute error}
\newacronym{rmse}{RMSE}{root mean squared error}
\newacronym{nrmse}{nRMSE}{normalized root mean squared error}
\newacronym{mse}{MSE}{mean squared error}
\newacronym{kld}{KLD}{Kullback-Leibler Divergence}
\newacronym{pv}{PV}{photovoltaic}
\newacronym{wrt}{w.r.t.}{with respect to}
\newacronym{pdf}{PDF}{probability density function}
\newacronym{mtl}{MTL}{multi-task learning}
\newacronym{stl}{STL}{single-task learning}
\newacronym{sps}{SPS}{soft parameter sharing}
\newacronym{hps}{HPS}{hard parameter sharing}
\newacronym{csn}{CSN}{cross-stitch network}
\newacronym{sn}{SN}{sluice network}
\newacronym{ern}{ERN}{emerging relation network}
\newacronym{nlp}{NLP}{natural language processing}
\newacronym{lstm}{LSTM}{long-tem short memory}
\newacronym{tcn}{TCN}{temporal convolution network}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{tl}{TL}{transfer learning}
\newacronym{dtw}{DTW}{dynamic time warping}
\newacronym{elbo}{ELBO}{expected lower bound}
\newacronym{csge}{CSGE}{coopetitive soft gating ensemble}
\newacronym{ae}{AE}{autoencoder}
\newacronym{cnnae}{CAE}{convolutional autoencoder}
\newacronym{vae}{VAE}{variational autoencoder}
\newacronym{dae}{DAE}{denoising autoencoder}
\newacronym{pca}{PCA}{principal component analysis}
\newacronym{rl}{RL}{representation learning}
\newacronym{sgd}{SGD}{stochastic gradient decent}
\newacronym{ttl}{TTL}{transductive transfer learning}
\newacronym{itl}{ITL}{inductive transfer learning}
\newacronym{sqtl}{SQTL}{sequential transfer learning}
\newacronym{aic}{AIC}{Akaike information criterion}
\newacronym{bic}{BIC}{Bayesian information criterion}
\newacronym{bma}{BMA}{Bayesian model averaging}
\newacronym{elm}{ELM}{extreme learning machine}
\newacronym{belm}{BELM}{Bayesian extreme learning machine}
\newacronym{relu}{ReLU}{Rectified Linear Unit}
\newacronym{DBN}{DBN}{deep belief network}
\newacronym{RBM}{RBM}{restricted Boltzmann machines}
\newacronym{RBF}{RBF}{radial-basis function}
\newacronym{blr}{BLR}{Bayesian linear regression}
\newacronym{sp}{SP}{source parameters}
\newacronym{crps}{CRPS}{continuous ranked probability score}


==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/custom_commands.tex <==

\newcommand{\todobox}[1]{\color{red}{TODO:~#1~}\color{black}}
\newcommand{\cn}{{[\color{red}\texttt{CitationNeeded}]}}
\newcommand{\sn}{{[\color{red}\texttt{SectionNeeded}]}}
\newcommand{\an}{[\texttt{AppendixNeeded}]}
\newcommand{\un}{[\texttt{URLNeeded}]}
\newcommand{\fn}{[\texttt{FigNeedded}]}
\newcommand{\en}{[\texttt{Eq.Needded}]}
\newcommand{\CN}[1]{{\color{red}[\texttt{Cite  #1}]}}
\newcommand{\subsubsubsection}[1]{~\\\noindent\textbf{#1}}
\newcommand\SEC[1]{Section~\ref{#1}} % replace with Sec. for a short version
\newcommand\DEF[1]{Def.~\ref{#1}}
% \newcommand\FIG[1]{\figurename~\ref{#1}} % replace with Fig. for a short version
\newcommand\FIG[1]{Fig.~\ref{#1}} % replace with Fig. for a short version
\newcommand\TBL[1]{Table~\ref{#1}} 
\newcommand\TBLs[1]{Tables~\ref{#1}}
\newcommand\EQ[1]{Eq.~\ref{#1}} % replace with Eq.. for a short version
\newcommand{\baseline}{\texttt{baseline}~}
\newcommand{\Baseline}{\texttt{Baseline}~}
\newcommand{\baselineNS}{\texttt{baseline}}
\newcommand{\WO}{\texttt{WINDOPEN~}}
\newcommand{\WS}{\texttt{WINDSYN~}}
\newcommand{\WR}{\texttt{WINDREAL~}}
\newcommand{\PO}{\texttt{PVOPEN~}}
\newcommand{\PS}{\texttt{PVSYN~}}
\newcommand{\PR}{\texttt{PVREAL~}}

\newcommand{\WONS}{\texttt{WINDOPEN}}
\newcommand{\WSNS}{\texttt{WINDSYN}}
\newcommand{\WRNS}{\texttt{WINDREAL}}
\newcommand{\PONS}{\texttt{PVOPEN}}
\newcommand{\PSNS}{\texttt{PVSYN}}
\newcommand{\PRNS}{\texttt{PVREAL}}


\newcommand{\PV}{\texttt{PV}~}
\newcommand{\WI}{\texttt{WIND}~}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/mathsymbols.tex <==
\opensymdef
\newsym[Size of input features.]{dimFeature}{D}
\newsym[The parameters of a linear model.]{parametersLinModel}{\boldsymbol{\theta}}
\newsym[All input features.]{inputFeatures}{\mathbf{X}}
\newsym[All response features.]{outputFeatures}{\mathbf{y}}
\newsym[A single input vector.]{inputFeatureVector}{\mathbf{x}}
\newsym[A single response respective target.]{outputFeatureVector}{y}
\newsym[A single response prediction.]{outputPredictionVector}{\hat{y}}
\newsym[The set of input features.]{setInputFeatures}{X}
\newsym[The set of response features.]{setOutputFeatures}{Y}
\newsym[Input feature space.]{inputFeatureSpace}{\mathcal{X}}
\newsym[Output feature space.]{outputFeatureSpace}{\mathcal{Y}}
\newsym[The number of samples.]{nSamples}{N}
\newsym[Index of samples.]{indexSamples}{n}
\newsym[Set of all real numbers.]{realNumber}{\mathbb{R}} 
\newsym[Set of all non-negative real numbers.]{realNumberNonNeg}{\mathbb{R}^{+}}
\newsym[Set of all positive real numbers.]{realNumberPos}{\mathbb{R}_{\geq 1}} 
\newsym[Set of all natural numbers.]{naturalNumber}{\mathbb{N}} 
\newsym[Set of all non-negative natural numbers.]{naturalNumberNonNeg}{\mathbb{N}^{+}} 
\newsym[Set of all positive natural numbers.]{naturalNumberPos}{\mathbb{N}_{\geq 1}}
\newsym[Normal distribution.]{normalDist}{\mathcal{N}} 
\newsym[A task.]{task}{\mathcal{T}} 
\newsym[The set of all tasks.]{allTasks}{\mathbb{T}} 
\newsym[Similarity measure between two task.]{similarityMeasure}{\mathcal{S}} 
\newsym[Precision matrix of a linear model.]{precisionMatrix}{\mathbf{S}} 
\newsym[Index of a source model.]{indexSourceModel}{m} 
\newsym[The number of source models.]{numberSourceModels}{M} 
\newsym[The dimension of the target.]{dimensionTarget}{I} 
\newsym[The index of the target task.]{indexTargetTask}{T} 
\newsym[CSGE weight not normalized.]{csgeWeightUnnormalized}{\bar{w}} 
\newsym[CSGE weight normalized.]{csgeWeightNormalized}{w} 
\closesymdef




==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec_itl_selection_conclusion}
We successfully evaluated several combinations of models, model selection, adaptation strategies, and two combination strategies on six datasets.
Our study's exhaustive evaluation is the most extensive evaluation for transfer learning in renewable power forecasts on real-world datasets.
We found that fine-tuning the final layer of a neural network, a well-known strategy, does not lead to convincing results in this setting.
Instead, replacing the layer with a Bayesian linear regression model trained with features extracted from the source and limited power measurements from the target task yields one of the best results, especially for a temporal convolutional neural network.
This result is best explained as source models in computer vision tasks are typically trained on many variations, e.g., various classification tasks. 
In contrast, renewable energy models are often trained on a single forecasting task.
This approach seems to generalize insufficiently for fine-tuning.
We suggest utilizing the forecast error with less than 30 days of training data for source model selection; the evidence is recommended with additional data.
We also showed how combining models leads to further significant improvements compared to considering a single model. 
The proposed coopetitive soft-gating ensemble combines source models solely based on the error of the target.
Our suggestion to utilize the Bayesian model averaging as an ensemble strategy is beneficial for minimal historical data.
To overcome the shortcomings of fine-tuning caused by limited data, we aim to augment the target data with synthetic data in the future. 
Likewise, we will expand our analysis for multi-task problems.


==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/experiment.tex <==
% \subsection{Experimental Results}
\section{Experimental Evaluation}
\label{sec_itl_selection_experiment}


% TODO THESIS
In the following~\SEC{sec_model_selection_doe}, we summarize the experimental setup.
We conduct experiments on six datasets with a total of $667$ parks.
Due to the utilized cross-validation, each park is once a target park.
Thereby, we provide the most extensive study for~\ac{itl} for renewable power forecasts.

We evaluate models through the mean performance rank, calculated across parks within a dataset, to show significant improvements against the \baseline.
In the appendix, we provide additional results concerning the forecast error and comparison to results from~\cite{Schreiber2021}.
\SEC{sec_model_selection_model_selection_experiment} provides the details of our first experiment to answer research questions one and two.
The second experiment in~\SEC{sec_model_selection_model_combination_experiment} details our findings for research question three.

\subsection{Overall Experimental Setup}\label{sec_model_selection_doe}
The preprocessing of the data is aligned with~\cite{VogtSynData2022,Schreiber2021} to assure comparability with the current state of the art.
As source models, we considered a~\ac{belm},~\ac{mlp}, and a~\ac{tcn}.
To have a robust \baseline that generalizes well with a limited amount of data and is known to mitigate the effects of overfitting, we trained a~\ac{gbrt} for each target task identical to~\cite{VogtSynData2022}.

\subsubsection{Datasets:} We conducted all experiments for day-ahead forecasts, between $24$ and $48$ hours into the future.
All datasets, summarized in \TBL{tbl_dataset_summary}, have~\ac{nwp} features as inputs, e.g., wind speed, wind direction, air pressure, or radiation.
For all datasets, we align those weather forecasts with the historical power measurements as the response for day-ahead forecasts.
These input features are weather forecasts from the European center for medium-range weather forecasts (ECMWF) or the Icosahedral Nonhydrostatic-European Union (ICON-EU) weather model.
\begin{table*}[t]
    \centering
    \caption{Overview of the evaluated datasets.}\label{tbl_dataset_summary}
    \begin{tabular}{l|llllll}

        \textbf{Dataset}           & \#\textbf{parks} & \#\textbf{features} & \textbf{train}   & \textbf{mean}    & \textbf{resolution} & \textbf{NWP}   \\
                                   &                  &                     & \textbf{samples} & \textbf{samples} &                     & \textbf{model} \\
        \hline
        \PO~\cite{Schreiber2021}   & 21               & 47                  & 6336             & 8424             & hourly              & ECMWF          \\
        \PS~\cite{VogtSynData2022} & 114              & 20                  & 30385            & 14920            & 15-min              & ICON-EU        \\
        \PR                        & 42               & 25                  & 58052            & 19344            & 15-min              & ICON-EU        \\
        \WO~\cite{Schreiber2021}   & 45               & 13                  & 27724            & 26636            & 15-min              & ECMWF          \\
        \WS~\cite{VogtSynData2022} & 260              & 29                  & 33714            & 16678            & 15-min              & ICON-EU        \\
        \WR                        & 185              & 33                  & 36129            & 12092            & 15-min              & ICON-EU
    \end{tabular}
\end{table*}

In all datasets, we have varying amounts of input features, resolutions, and different numbers of samples for training and testing.
For instance, the \PO has $47$ features, where various manually engineered features take seasonal patterns of the sun into account.
In contrast, these manually engineered features are not included in other datasets.

Also note that four datasets, the \PONS, \WONS, \WSNS, and \PS have already been investigated, see e.g.~\cite{Schreiber2021,VogtSynData2022}.
This is not the case for \WR and \PRNS.
These two datasets are not publicly available.
However, they are the most realistic datasets due to their diversity.
The \WR dataset consists of 99 different nominal capacities, 13 turbine manufacturers, and six hub heights.
All parks are located in Germany.
PV power plants in the \PR dataset have 31 different nominal capacities, ten tilt orientations, and nine azimuth orientations and are also located in Germany.
It is also important to note that forecasting the expected power generation from wind parks is more challenging than for~\ac{pv} parks.
For additional insights on the challenges and the datasets refer to the~\ref{sec_appendix_model_selection_data}.

Each dataset was split through five-fold cross-validation so that \textit{each park is once a target task} and four times a source park.
We trained source models and their hyperparameters on the training and validation data.
We split the training into the four seasons for training target models and
limited the training data to $7,14,30,60$ or $90$ days of training data, respectively.
The presented results are mean values for all tasks and seasons.
This setup assures that results are not biased by seasonality~\cite{Jens2019}.
All input features of all datasets are normalized.
We normalized the historical power by the nominal power to make errors comparable.
We resampled all datasets to have a $15$-minute resolution except the \PO dataset, which we resampled for an hourly resolution due to the low initial resolution.
A predefined test set is given for the \WS and \PS datasets.
In the case of the \WO and \PONS, we used the first year's data as training data and the remaining data as test data, identical to~\cite{Schreiber2021}.
Due to this diversity in the number of historical power measurements for the \PR and \WR datasets, $25\%$ randomly sampled days are considered test data.
As each day is based on an independent day ahead~\ac{nwp} forecasts, no information is leaked from the future to the past~\cite{Gensler2018}.
We use $25\%$ of the remaining days for validation and the rest for training.

\subsubsection{Source Models}\label{sec_itl_experiment_source_models}
As pointed out earlier, due to the weather dependency for renewable power forecasts, the input features of the models are themselves forecasts from the ~\ac{nwp} model.
Respectively, we can directly utilize those to train, e.g., an~\ac{mlp} to forecast the expected power of the next day.
To optimize hyperparameters of those models, we utilize a tree-structured Parzen sampler for $200$ samples on the validation data.
Details of the chosen hyperparameters are provided in the~\ref{sec_appendix_model_selection_experiment}.

In total, we train four kinds of models.
The trained~\ac{belm} is particularly interesting as a source model because it can directly measure similarity by the evidence and has a linear increase in time for updating the model.
We train an~\ac{mlp} as it is common practice in the renewable power forecast industry~\cite{Schreiber2021}.
To account for cyclic behavior within the forecast, we also train a~\ac{tcn} architecture, similar to~\cite{Schreiber2021}.
To have a strong \baseline that generalizes well we trained a~\ac{gbrt}~\cite{VogtSynData2022}.

\subsubsection{Evaluation Method}
We calculated the error on the test dataset through the~\ac{nrmse} through~\EQ{eq_nrmse} for all combinations of seasons and available training data.
For a given dataset, season, and the number of days of training data, we calculated the mean performance rank based on the~\ac{nrmse}.
We test for a significant improvement compared to the \baseline by the Wilcoxon test ($\alpha = 0.01$) across all parks within a dataset.

\begin{table*}[!ht]
    \centering
    \caption{Rank summary for all models, selections, and adaptation strategies on the PV datasets, cf.~\TBL{tbl_model_selection_overview}. Only those within the top four ranks for a dataset are included. GBRT is the \baseline and all models are tested if the forecasts error is significantly ($\alpha=0,01$) better ($\vee$), worse ($\wedge$), or not significantly different ($\diamond$). We conduct this hypothesis test for all parks within a dataset for the given number of days training data. The colors denote the respective rank. Blue indicates a smaller (better) rank and red a higher (worse) rank.}\label{tbl_model_selection_rank_pv}
    \includegraphics[width=0.92\textwidth,trim=0.1cm 0.09cm 0.0cm 0cm, clip]{sections/inductive_transfer_learning/selection_and_ensembles/tables/stl_rank_pv}
\end{table*}
\begin{table*}[!ht]
    \centering
    \caption{Rank summary for all source models, selections, and adaptation strategies on the wind datasets. Cf.~\TBLs{tbl_model_selection_overview} and~\ref{tbl_model_selection_rank_pv}.}\label{tbl_model_selection_rank_wind}
    \includegraphics[width=0.92\textwidth,trim=0.1cm 0.09cm 0.0cm 0cm, clip]{sections/inductive_transfer_learning/selection_and_ensembles/tables/stl_rank_wind}
\end{table*}
\begin{table*}[!ht]
    \centering
    \caption{Rank summary of ensembles on the PV datasets. The best model, the TCN-EV-DILI, from the experiment in ~\SEC{sec_model_selection_model_selection_experiment} is the baseline. Cf.~\TBLs{tbl_model_selection_overview} and~\ref{tbl_model_selection_rank_pv}.}\label{tbl_model_selection_rank_pv_ensemble}
    \includegraphics[width=0.92\textwidth,trim=0.1cm 0.09cm 0.0cm 0cm, clip]{sections/inductive_transfer_learning/selection_and_ensembles/tables/ensemble_rank_pv}
\end{table*}
\begin{table*}[!ht]
    \centering
    \caption{Rank summary of ensembles on the wind datasets. Cf.~\TBL{tbl_model_selection_rank_pv_ensemble}.}\label{tbl_model_selection_rank_wind_ensemble}
    \includegraphics[width=0.92\textwidth,trim=0.1cm 0.09cm 0.0cm 0cm, clip]{sections/inductive_transfer_learning/selection_and_ensembles/tables/ensemble_rank_wind}
\end{table*}
\begin{table*}[!ht]
    \centering
    \caption{Mean nRMSE of ensembles on the PV datasets. The best model, the TCN-EV-DILI, from the experiment in ~\SEC{sec_model_selection_model_selection_experiment} is the baseline. Cf.~\TBLs{tbl_model_selection_overview} and~\ref{tbl_model_selection_rank_pv}.}\label{tbl_model_selection_rmse_pv_ensemble}
    \includegraphics[width=0.92\textwidth,trim=0.1cm 0.09cm 0.0cm 0cm, clip]{sections/inductive_transfer_learning/selection_and_ensembles/tables/ensemble_rmse_pv}
\end{table*}
\begin{table*}[!ht]
    \centering
    \caption{Mean nRMSE of ensembles on the wind datasets. Cf.~\TBL{tbl_model_selection_rmse_pv_ensemble}.}\label{tbl_model_selection_rmse_wind_ensemble}
    \includegraphics[width=0.92\textwidth,trim=0.1cm 0.09cm 0.0cm 0cm, clip]{sections/inductive_transfer_learning/selection_and_ensembles/tables/ensemble_rmse_wind}
\end{table*}

\setcounter{question}{0}
\subsection{Experiment on Model Selection and Model Adaptation}\label{sec_model_selection_model_selection_experiment}
This section conducts an experiment to answer research questions one and two simultaneously as a model selection technique can only be evaluated after the adaptation:
% ``What is an appropriate similarity measure for model selection for a new target park from a model-hub with pre-trained models?'' and ``What is the best adaptation strategy once a model is selected?''\todobox{as definition like in the intro}
\begin{question}
    What is an appropriate similarity measure for model selection for a new target park from a model hub with pre-trained models?
\end{question}
\begin{question}
    What is the best adaptation strategy once a model is selected?
\end{question}


\subsubsection{Findings Questions 1 \& 2}
Model selection and adaptation strategies highly influence each other. With limited training data, between $7$ and $30$ days, selecting a model based on the forecast error with no adaptation has one of the best results. Replacing the final layer by a~\ac{blr} is superior with additional data.
None of the fine-tuning methods is among the best models.

\subsubsection{Experimental Setup}
The source models are those detailed in~\SEC{sec_itl_experiment_source_models}.
As adaptation strategies, we consider those mentioned in~\SEC{sec_itl_selection_method_adaption}.
For fine-tuning, we train for a single epoch and optimize hyperparameters through grid search on $30\%$ of the available target data.
% Hyperparameters of the fine-tuning adaptation strategies are optimized through a grid-search based on $30\%$ of the available target data.
% Adaptations utilizing fine-tuning, such as weight decay, are defined in~\SEC{sec_itl_selection_method_adaption}.

For the weight decay adaptation, we optimize seven logarithmically spaced learning rates between $10^{-1}$ and $10^{-4}$, similar to~\cite{You2021LogMe}.
We take seven grid points for the amount of penalty $\lambda$ in the logarithmic space between $10^{-6}$ to $10^{-3}$, similar to~\cite{You2021LogMe}.
We use the same learning rate for the Bayesian tunning and weight decay source.
The amount of penalty $\lambda$ for the $L_{\text{Bayesian}}$ loss is one of $[0.1, 0.25, 0.5, 1, 2, 4, 8]$.
$\lambda$ is one of $[1, 0.1]$ for the weight decay source.
Note that during the training, we shuffle the data.
For other approaches, hyperparameter optimization is not required.

\subsubsection{Detailed Findings}

Results of the best techniques are summarized in~\TBL{tbl_model_selection_rank_pv} and \ref{tbl_model_selection_rank_wind}.
We only show models appearing at least once within the top four ranks for a dataset.
The~\ac{belm} is among the best models and outperforms the \baseline up to $30$ days of training data.
With less or equal than $14$ days of training data, it seems beneficial to directly utilize a model without any model adaptation.
Starting with $30$ days of training data utilizing a~\ac{blr} trained on extracted features from the source model and the historical power from the target is beneficial, especially for \WR and \PRNS.
This effect occurs as features extracted from a single model from a single prediction task do not generalize well enough for other parks.
Therefore a sufficient amount of data is required to train the~\ac{blr} to compensate for differences between a source and a target park.

These two observations let us conclude with two critical considerations for real-world applications.
First, due to the learning procedure of the gradient descent, there is a high risk of catastrophic forgetting that should be avoided for model hubs in safety-critical areas such as renewable power forecasts.
Second, the~\ac{blr} gives rise to optimal training due to the convex optimization problem, which reduces the risk of catastrophic forgetting.
Notably, neither a weight decay nor the Bayesian tuning adaptation strategy is within the best models in the evaluated scenarios.
This observation is surprising as this fine-tuning approach is common in various domains.
However, due to the source model's training on a single park approach, there is a high risk that even the best-selected source model causes catastrophic forgetting as the model is too specific.
For instance, catastrophic forgetting may appear due to slightly different weather conditions or physical characteristics such as the turbine type.

An additional study given in the~\ref{sec_appendix_exp_model_selection_and_adaption} shows that for fine-tuning techniques, the evidence selection strategy is superior for the~\ac{tcn} model regardless of the adaptation strategy.
For the~\ac{mlp}, a selection through the~\ac{nrmse} is preferable.
Most likely, the probabilistic approach of the evidence and, therefore, the more comprehensive treatment of similarity better captures the correlations between source and target for the convolutional layers in the~\ac{tcn}.
To update the weights of the final layer of the~\ac{mlp} the~\ac{nrmse} is sufficient.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Ablation Study}

% \todobox{we could fix on one selection strategy and compare the result, e.g., for 60 days of training data}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experiment on Model Combination}\label{sec_model_selection_model_combination_experiment}
In this section, we conduct an experiment to answer research question three.
% ``Are ensemble strategies beneficial to combine knowledge compared to selecting and adapting a single model?''
\begin{question}
    Compared to selecting and adapting a single model, are ensemble strategies beneficial for combining knowledge?
\end{question}

\subsubsection{Findings Research Question 3}
Ensembles improve results from the previous experiment significantly. For more straightforward problems, an approach utilizing~\ac{bma} is preferable. For more complex scenarios, an approach by the~\ac{csge} is superior.

\subsubsection{Experimental Setup}
% The best model from the previous experiment, the \textit{TCN-EV-DILI}, is the \baselineNS.
% We combine models through~\ac{bma} and~\ac{csge}.
% The~\ac{bma} considers one of the source model types as ensemble members.
% For the neural networks, we replace the last layer with the~\ac{blr}. 
% The~\ac{belm} is updated directly with the target data.
% The first variant of the~\ac{csge} utilizes source models without adaptation.\todobox{add names}
% The second one replaces the final layer by the~\ac{blr}\todobox{add names}.
% We consider one variant where the~\ac{gbrt} from the previous experiment is included as the source model\todobox{add names}.
% All three variants are evaluated for the~\ac{mlp} and the~\ac{tcn} source models.
% \todobox{check content}
The best model, the TCN-EV-DILI, from the experiment in ~\SEC{sec_model_selection_model_selection_experiment} is the \baseline.
For the~\ac{bma}, we first update all source models based on available target data as previously described.
For the~\ac{mlp} and~\ac{tcn} source models we replace the final layer through~\ac{blr} model(s), as detailed for the direct linear adaptation.
After this adaptation for the target, each model provides a predictive posterior distribtion according to~\EQ{eq_lin_predictive_posterior} that is combined by~\ac{bma} with~\EQ{eq_bayesian_model_averaging}.
We consider three variants for the~\ac{bma}, one for each of the three source model types.

For the~\ac{csge}, we calculate the global and forecast horizon-dependent error based on the~\ac{nrmse}.
We estimate the local error through a k-nearest neighbor approach.
Therefore, we first reduce the dimension of the feature space through~\ac{pca} to two components.
We consider three neighbors within this reduced features space to estimate the local error in the features space.
The hyperparameter $\eta$ is selected as either one or two through grid-search.
In total, we consider six variants of the~\ac{csge}:
Two for the~\ac{mlp} and~\ac{tcn} model where the source models are not updated for the target (CSGE-MLP-DI/CSGE-TCN-DI), two variants, where the final layer of the~\ac{mlp} and~\ac{tcn} source models are updated through~\ac{blr} (CSGE-MLP-DILI/CSGE-TCN-DILI), and these two variants are extended, where we utilize the~\ac{gbrt} as an additional source model (CSGE-MLP-DILI-GBRT/CSGE-TCN-DILI-GBRT).

\subsubsection{Detailed Findings}

Results are summarized in~\TBLs{tbl_model_selection_rank_pv_ensemble} and~\ref{tbl_model_selection_rank_wind_ensemble}.
For the~\ac{pv} datasets, the best~\ac{csge} variants outperform the \baseline in almost all cases.
At the same time, the~\ac{bma} achieves excellent results for the \PO dataset and the \PR dataset for up to 30 days of training data.
With minimal data, less than 30 days, the~\ac{bma} is among the best for the wind datasets.
With more training data, the~\ac{csge} with~\ac{tcn} source models, where the final layer is replaced by~\ac{blr} is the best.
We can also observe for these datasets that additionally considering the~\ac{gbrt} as the source model improves the results.

This observation also shows the flexibility of the~\ac{csge}.
Due to the combination through the forecast error, we can combine arbitrary models.
This flexibility is not given by the proposed~\ac{bma} approach.
However, the~\ac{bma} has the advantage that probabilistic forecasts are provided, which are not the focus of this article, but their evaluation is given in the appendix.

Another important consideration is that in almost all cases, the ensemble techniques outperform the~\baselineNS, which is the best model from the previous experiment.
These results show that a single source model's selection and adaptation process is highly uncertain because the model may be too specific for the target.
Due to specific characteristics of a single model, for example, the weather at the location or technical characteristics, selecting and adapting a single source model for the target is challenging.
In contrast, the combination of several models probably has a balancing effect on individual properties and improves the error significantly.

Besides the previous statistical discussion through the mean performance ranking, we also need to include an analysis of the forecast error for real-world implications.
Therefore, the forecast error, by means of the mean nRMSE, is summarized for this experiment in~\TBLs{tbl_model_selection_rmse_pv_ensemble} and \ref{tbl_model_selection_rmse_wind_ensemble}.
The best model from the previous experiment is again the \baselineNS.

In these tables, the error of the models decreases with increasing training data amount for all six datasets.
For the PV datasets, the best model has the largest error for the \PR dataset.
The best forecast error for this dataset is only $9.8$ percent with seven days of training data.
For the \PO with seven days of training data, the error is with $7$ percent error rate lower than results from~\cite{Schreiber2021}.

Also, for the~\WO dataset, the best models have similar error rates, between $16.3$ for seven days and $13.8$ percent for $90$ days of training data, similar to the result in~\cite{Schreiber2021}
The \WS dataset has the largest errors, between $16.7$ and $14.6$ percent, for the wind datasets.

Based on the analysis of the nRMSE, we can observe that even with a small amount of training data, good up to excellent prediction quality can be achieved. Furthermore, the mean nRMSE with more than 30 days often corresponds to error rates with a whole year of training data~\cite{Schreiber2021, VogtSynData2022}.

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/figures/bayesian_model_selection.tex <==
{
\Large
\resizebox{0.39\textwidth}{!}{%
    \begin{tikzpicture}

        \draw[very thick,-] (0,0) -- (10.5,0) node[anchor=north] {$\mathcal{D}$};
        \draw[very thick,->] (5,0) -- (5,5.5) node[anchor=south west, yshift=-1cm] {Evidence};

        \filldraw[draw=black,fill=lightgray, fill opacity=0.2] (4.5,0) rectangle (5.5,4) ;
        \draw[thick,<->] (4.5,-0.5) -- (5.5,-0.5) node[anchor=north east] {$\mathcal{D}_T$};
        \node at (6.5,3.5) {$p(\mathcal{D}|M_1)$};


        \filldraw[draw=black,fill=blue, fill opacity=0.2] (1.5,0) rectangle (8.5,1) ;
        \node at (2.2,1.3) {$p(\mathcal{D}|M_2)$};

    \end{tikzpicture}
}
}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/figures/blended_learning.tex <==
\resizebox{0.95\textwidth}{!}{%
    \begin{tikzpicture}

        \draw[thick,->] (0,0) -- (10.5,0) node[anchor=north, xshift=-8.5cm, yshift=-0.1cm] {available training data};
        \draw[thick,->] (0,0) -- (0,5.5) node[anchor=south west, yshift=-3.75cm, xshift=-0.1cm, rotate=90] {weighting};

        %\draw[step=1cm,gray,very thin] (0, 0) grid (10, 5);

        \draw[color=black,dashed, thick] (0,0) .. controls (10,0) and (3,4.5) .. (10,4.9) node[anchor=south, xshift=-1cm] {target model};
        \draw[color=black,dotted, thick] (0,0) .. controls (2.5,0) and (2.5,5) .. (5,5) node[anchor=south] {'Blended Transfer'};
        \draw[color=black,dotted, thick] (5,5) .. controls (7.5, 5) and (7.5, 0) .. (10,0.1);
        \draw[color=black, dash dot, thick] (0,5) .. controls (5, 5) and (0,0) .. (10, 0) node[anchor=south, xshift=-8.5cm, yshift=5cm] {source models};


    \end{tikzpicture}
}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/figures/overview_csge.tex <==
{
    \large
    \begin{center} 
    \resizebox{0.75\textwidth}{!}{%
        \tikzstyle{block} = [rectangle, rounded corners, text centered, draw=black]
        \tikzstyle{clear} = [rectangle, rounded corners, text centered]
        \tikzstyle{arrow} = [thick,->,>=stealth]
        \tikzstyle{connect} = [thick,-,>=stealth]
        % 
            \begin{tikzpicture}[node distance=1cm]
            
            \node [block, text width=2cm, text height=6cm,] (cw) {};
            \node [block, text width=2cm, text height=6cm, right of=cw, xshift=2.5cm] (nw) {};
            \node [block, text width=2cm, text height=6cm, right of=nw, xshift=4cm] (ap) {};
            \node[text width=2.6cm] at (0.3,0.0) {\textbf{Compute Weights}};
            \node[text width=2.6cm] at (3.75,0.0) {\textbf{Normalize Weights}};
            \node[text width=2.3cm] at (8.6,0.0) {\textbf{Aggregate Forecasts}};
            
            
            \node [block, text width=1.5cm, text height=0.25cm, above of=cw, opacity=0.75, yshift=1.75cm, dashed] (global) {Global};
            \node [block, text width=1.5cm, text height=0.25cm, below of=global, opacity=0.75, yshift=-0.5cm, dashed] (local) {Local};
            \node [block, text width=1.5cm, text height=0.25cm, below of=local, opacity=0.75, yshift=-1.8cm, dashed] (fh) {Forecast Horizon};
            
            \node [block, text width=3cm, text height=0.5cm, left of=cw, xshift=-3cm, yshift=2.7cm] (sm1) {Source Model (1)};
            \node [block, text width=3cm, text height=0.5cm, below of=sm1, yshift=-0.5cm] (sm2) {Source Model (2)};
            \node [clear, text width=3cm, text height=0.5cm, below of=sm2, yshift=-0.5cm] (sdots) {...};
            \node [block, text width=3cm, text height=0.5cm, below of=sdots, yshift=-0.5cm] (smj) {Source Model (M)};
            
            \node [clear, text width=0.5cm, text height=0.5cm, left of=cw, xshift=-6.5cm] (x) {};
            \node [clear, text width=0.0cm, text height=0.0cm, right of=x] (xa) {};
            \draw [connect] (x.east) -- node[anchor=north, yshift=0.6cm, xshift=-0.25cm] {$\inputFeatureVector_{t + k | t}$} (xa.east);
            \draw [arrow] (xa.east) |- node[] {} (sm1);
            \draw [arrow] (xa.east) |- node[] {} (sm2);
            \draw [arrow] (xa.east) |- node[] {} (smj);
            
            \node [clear, text width=0.5cm, text height=0.5cm, right of=ap, xshift=2cm] (y) {};
            \draw [arrow] (ap.east) -- node[anchor=north, yshift=0.75cm] {$\bar{\outputPredictionVector}_{t+k|t}$} (y.west);
            
            \node [clear, right of=sm1, xshift=3cm, text width=2cm] (cw1) {};
            \node [clear, right of=sm2, xshift=3cm, text width=2cm] (cw2) {};
            \node [clear, right of=smj, xshift=3cm, text width=2cm] (cwj) {};
            \draw [arrow] (sm1.east) -- node[anchor=north, yshift=0.8cm] {$\outputPredictionVector^{(1)}_{t+k|t}$} (cw1.west);
            \draw [arrow] (sm2.east) -- node[anchor=north, yshift=0.8cm] {$\outputPredictionVector^{(2)}_{t+k|t}$} (cw2.west);
            \draw [arrow] (smj.east) -- node[anchor=north, yshift=0.8cm] {$\outputPredictionVector^{(\numberSourceModels)}_{t+k|t}$} (cwj.west);
            
            \node [clear, right of=cw1, xshift=2.5cm, text width=2cm] (nw1) {};
            \node [clear, right of=cw2, xshift=2.5cm, text width=2cm] (nw2) {};
            \node [clear, right of=cwj, xshift=2.5cm, text width=2cm] (nwj) {};
            \draw [arrow] (cw1.east) -- node[anchor=north, yshift=0.8cm] {$\csgeWeightUnnormalized^{(1)}_{t+k|t}$} (nw1.west);
            \draw [arrow] (cw2.east) -- node[anchor=north, yshift=0.8cm] {$\csgeWeightUnnormalized^{(2)}_{t+k|t}$} (nw2.west);
            \draw [arrow] (cwj.east) -- node[anchor=north, yshift=0.8cm] {$\csgeWeightUnnormalized^{(\numberSourceModels)}_{t+k|t}$} (nwj.west);
            
            \node [clear, right of=nw1, xshift=4cm, text width=2cm] (ap1) {};
            \node [clear, right of=nw2, xshift=4cm, text width=2cm] (ap2) {};
            \node [clear, right of=nwj, xshift=4cm, text width=2cm] (apj) {};
            \draw [arrow] (nw1.east) -- node[anchor=north, yshift=0.8cm] {$\csgeWeightNormalized^{(1)}_{t+k|t} \cdot \outputPredictionVector^{(1)}_{t+k|t}$} (ap1.west);
            \draw [arrow] (nw2.east) -- node[anchor=north, yshift=0.8cm] {$\csgeWeightNormalized^{(2)}_{t+k|t} \cdot \outputPredictionVector^{(2)}_{t+k|t}$} (ap2.west);
            \draw [arrow] (nwj.east) -- node[anchor=north, yshift=0.8cm] {$\csgeWeightNormalized^{(\numberSourceModels)}_{t+k|t} \cdot \outputPredictionVector^{(\numberSourceModels)}_{t+k|t}$} (apj.west);
            
            \node [clear, right of=sm1, xshift=1.25cm] (sc1) {};
            \node [clear, right of=cw1, xshift=2.5cm, yshift=-0.5cm, text width=2cm] (nw1h) {};
            \draw [arrow, opacity=0.5] (sc1.center) |- node[] {} (nw1h.west);
            \node [clear, right of=sm2, xshift=1.25cm] (sc2) {};
            \node [clear, right of=cw2, xshift=2.5cm, yshift=-0.5cm, text width=2cm] (nw2h) {};
            \draw [arrow, opacity=0.5] (sc2.center) |- node[] {} (nw2h.west);
            \node [clear, right of=smj, xshift=1.25cm] (scj) {};
            \node [clear, right of=cwj, xshift=2.5cm, yshift=-0.5cm, text width=2cm] (nwjh) {};
            \draw [arrow, opacity=0.5] (scj.center) |- node[] {} (nwjh.west);
            
            \node [clear, text width=3cm, text height=0.5cm, right of=sdots, xshift=1.25cm] (ydots) {...};
            \node [clear, text width=3cm, text height=0.5cm, right of=sdots, xshift=4.75cm] (wdots) {...};
            \node [clear, text width=3cm, text height=0.5cm, right of=sdots, xshift=9cm] (wydots) {...};
            
            
            \end{tikzpicture}
        % %
    }
    \end{center}
}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/figures/selection_and_combination.tex <==
{
\huge

\tikzstyle{block} = [rectangle, rounded corners, minimum width=3.5cm, minimum height=2cm,text centered, text width=5cm, draw=black]
\tikzstyle{block2} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, text width=3cm, draw=black]
\tikzstyle{cbox} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black]

\begin{tikzpicture}[node distance=1.5cm]
    % \centering
    \tikzstyle{arrow} = [ultra thick,->,>=stealth]

    \node (sd) [xshift=0cm] {};
    \node (comb) [block, below of=sd, right of=sd, , xshift=3cm, yshift=-4cm, rotate=90, text width=8cm] {1.~Selection and 2.~Adaption and 3.~Combination};

    \node (m1) [block2, left of=comb, below of=sd, xshift=1.5cm, yshift=-1.5cm, color=orange, text width=3.3cm] {Model $\mathcal{T}_1$};
    \node (m2) [block2, below of=m1, color=darkgreen, text width=3.3cm] {Model $\mathcal{T}_2$};
    \node (m3) [block2, below of=m2, color=gray, text width=3.3cm] {Model $\mathcal{T}_M$};
    \node (m4) [block2, below of=m3, yshift=-1cm, color=red, text width=3.3cm] {Model $\mathcal{T}_T$};

    \draw [arrow] (sd) -| node[] {} (comb);

    \draw [ultra thick] (-4.5, -13) |- node[] {} (sd.east);
    \draw [arrow] (-4.5, -13) -| node[] {} (comb.west);

    \draw [arrow] (m1.east) -- node[] {} (3.5, -3);
    \draw [arrow] (m2.east) -- node[] {} (3.5, -4.5);
    \draw [arrow] (m3.east) -- node[] {} (3.5, -6);
    \draw [arrow] (m4.east) -- node[] {} (3.5, -8.5);

    \draw [arrow] (comb.south) -- node[anchor=east, yshift=0.6cm, xshift=1.4cm] {Forecast} (8.4, -5.5);

    \draw [arrow, ] (-5, -3) -- node[] {} (m1.west);
    \draw [arrow] (-5, -4.5) -- node[] {} (m2.west);
    \draw [arrow] (-5, -6) -- node[] {} (m3.west);
    \draw [arrow] (-5, -8.5) -- node[] {} (m4.west);

    \node (pv) [cbox, right of=m2, xshift=-7.5cm, yshift=-1cm, rotate=90, dashed, text width=8cm] {Input and Response Features};


    \node (bb) [cbox, xshift=0cm, yshift=-4.5cm, text width= 4cm, text height=4.5cm, draw=black, dashed] {};
    \node (ob) [cbox, xshift=0cm, yshift=-8.5cm, text width= 4cm, text height=2cm, draw=black, dashed] {};

    \node (sm) [above of=bb, yshift=1.3cm, color=black] {Model Hub};
    \node (tm) [below of=ob, yshift=-0.5cm, color=black] {Target Model};

    \node (dots1) [below of=m2, yshift=0.75cm] {...};

    \draw[black,fill=black] (-4.5, -3) circle (.5ex);
    \draw[black,fill=black] (-4.5, -4.5) circle (.5ex);
    \draw[black,fill=black] (-4.5, -6) circle (.5ex);
    \draw[black,fill=black] (-4.5, -8.5) circle (.5ex);

\end{tikzpicture}
}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/figures/similarity_wind_example.tex <==
{
\Large
% \resizebox{\textwidth}{!}{%
\begin{tikzpicture}
	\begin{axis}%
		[
			grid=minor,
			xmin=0,
			xmax=20,
			axis x line=bottom,
			ytick={0,0.2,...,1.0},
			ymax=1.1,
			axis y line=left,
		]
		\addplot%
		[
			orange,%
			mark=none,
% 			dashed,
			mark options={scale=4},
			opacity=0.5,
			samples=100,
			domain=-0:20,
		]
		(x,{1/(1+exp(-x+5))});
		\addplot%
		[
			red,%
			mark=none,
			samples=100,
			mark options={scale=4},
			xticklabels={\empty},
			yticklabels={\empty},
			domain=-0:20,
		]
		(x,{10/(10+exp(-x+10))});
		\addplot%
		[
			darkgreen,%
			mark=none,
% 			dashed,
			mark options={scale=4},
			opacity=0.5,
			samples=100,
			xticklabels={\empty},
			yticklabels={\empty},
			domain=-0:20,
		]
		(x,{0.5/(0.50+exp(-x*0.8+10))});
	\end{axis}
   
	\node[text width=3.5cm,xshift=-0.5cm] at (4,-1)  {Wind Speed [$\frac{m}{s^2}$]};
	\node[text width=3cm] at (3.5,5.5)  {{\large \color{orange} $\mathbb{E}[p(\setOutputFeatures_{1}|\setInputFeatures_{1}, \parametersLinModel_{1})]$}};
	\node[text width=3cm, text=red] at (6.5,5.5)  {\large $\mathbb{E}[p(\setOutputFeatures_{T}|\setInputFeatures_{T}, \parametersLinModel_{T})]$};
	\node[text width=3cm, text=gray] at (7.5,4.5)  {{\large \color{darkgreen} $\mathbb{E}[p(\setOutputFeatures_{2}|\setInputFeatures_{2}, \parametersLinModel_{2})]$}};

	\node[text width=5cm, rotate=90, yshift=0.25cm] at (-1,3.5)  {Normalized Power~[-]};

	\draw [stealth-stealth](1.75,2.5) -- (2.6,2.5) ;
	\node[text width=3cm] at (2.6,2.8)  {\large $\similarityMeasure({\color{orange} \mathcal{T}_1}, {\color{red} \mathcal{T}_T})$};

	\draw [stealth-stealth](2.65,2.5) -- (4.55,2.5) ;
	\node[text width=3cm] at (4.6,2.8)  {\large $\similarityMeasure({\color{darkgreen} \mathcal{T}_2}, {\color{red} \mathcal{T}_T})$};
	
\end{tikzpicture}

}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/introduction.tex <==
% \subsection{Ensembles and Model Selection}
%TODO THESIS
\section{Introduction}
% One fundamental problem in renewable power forecasts is adding new parks to an operator's portfolio with the extension of volatile energy resources, such as wind and~\ac{pv} parks.
With the extension of volatile energy resources, such as wind and~\ac{pv} parks, one fundamental problem is adding new parks to an operator’s portfolio.
The historical data for such a new (target) park is often limited.
At the same time, reliable forecasts are fundamental to assure grid stability due to the weather dependency.
However, typically there are numerous pre-trained models from existing parks that we can utilize for such a forecasting task~\cite{Schreiber2019a}.
Utilizing those pre-trained source models often increases the forecast accuracy, reduces the computational effort, and reduces the carbon emission for training a new model~\cite{Schwartz2019,Schreiber2021}.
Now, the question arises \textit{what is the best way to use} of this \textit{model hub} of pre-trained models.
The field of research~\ac{itl} provides methods for this problem~\cite{You2021LogMe}.

\begin{figure*}[tb]\centering
\subfloat[Process of model selection, adaptation, and combination.\label{fig_model_selection_and_adaption}]{
\scalebox{0.38}{
\input{sections/inductive_transfer_learning/selection_and_ensembles/figures/selection_and_combination}}}
\qquad
\subfloat[Similarity between sources $\task_1$ and $\task_2$ with a target task $\task_T$ for mean wind power predictions.\label{fig_task_sim_wind_example}]{
\scalebox{0.67}{
\input{sections/inductive_transfer_learning/selection_and_ensembles/figures/similarity_wind_example}}}
\caption{Diagrams illustrating the knowledge transfer based on a model hub.}
\end{figure*}
\FIG{fig_model_selection_and_adaption} summarizes our proposed strategy.
The first step is to select an appropriate source model.
Recently,~\cite{You2021LogMe,You2021Hub} showed that selecting an appropriate source model for knowledge transfer for a target substantially influences the test error for computer vision tasks.
To \textbf{select} a source model, consider, e.g., we have two source tasks $\task_1$ and $\task_2$ of a wind park with model parameters $\parametersLinModel_1$ and $\parametersLinModel_2$. 
These models have a set of input observations $\setInputFeatures_1$ and $\setInputFeatures_2$ as well as the sets of response values $\setOutputFeatures_1$ and $\setOutputFeatures_2$.
Based on this information, we want to select one of the models for knowledge transfer for a target task $\task_T$ with parameters $\parametersLinModel_T$ and its respective sets $\setInputFeatures_T$ and $\setOutputFeatures_T$.

The diagram in~\FIG{fig_task_sim_wind_example} visualizes this problem for wind power forecasts.
In renewable power forecasts, we utilize weather forecasts, such as the wind speed or radiation, from a so called~\ac{nwp} model.
These predicted weather features are the input $\setInputFeatures$ to \ac{ml} models, with parameters $\parametersLinModel$, predicting the expected power generation $\mathbb{E}[p(\setOutputFeatures|\setInputFeatures, \parametersLinModel)]$ in a \textit{day-ahead} forecasting task between $24$ and $48$ hours into the future.
In the diagram, we can observe that the similarity $\similarityMeasure$ depends on the relation between the input feature wind and the power generated by a wind park, i.e., for different wind speeds and models, we expect a different power generation.

Once a model is selected, the second step adapts the source knowledge with the limited target data with an~\textit{adaptation strategy}.
Often this adaptation strategy is fine-tuning the final layer of a neural network.
Only with such an adaptation can we make reliable and task-specific power forecasts for a new target task of a new park with limited data.
To the best of our knowledge, different adaptation and selection strategies have been so far not considered for~\ac{itl} in the field of renewable power forecasts.
We close this gap with this article.
Selecting and adapting a single source model from a model hub has the disadvantage of neglecting knowledge from other source tasks that are potentially beneficial.
However, we can additionally \textbf{combine} models through ensemble techniques.
Combining knowledge can be seen as a mixture of selection, where more relevant models are weighted higher, and adaptation, where source models are weighted to fit the target.
% We can circumvent this problem by ensemble strategies considering multiple source models for a target task.
% Such an ensemble technique is an \textit{model combination} strategy.
Since~\ac{itl} has been insufficiently studied so far for renewable power forecasts~\cite{Alkhayat2021}, especially for day-ahead forecast horizons between $24$ and $48$ hours into the future, we answer the following research questions:
\begin{question} 
What is an appropriate similarity measure for model selection for a new target park from a model hub with pre-trained models?
\end{question}
\begin{question} 
 What is the best adaptation strategy once a model is selected?
\end{question}
\begin{question} 
 Compared to selecting and adapting a single model, are ensemble strategies beneficial for combining knowledge?
\end{question}

To answer those research questions, we train a~\ac{belm}, a~\ac{mlp}, and a~\ac{tcn} as source models on six datasets including $667$ distinct parks.
We consider the~\ac{gbrt} as a \baseline that outperforms physical models even with limited target data~\cite{VogtSynData2022}.

Based on these datasets and source models, our main contributions to answering the research questions can be summarized as follows:
First, we propose the~\ac{nrmse}, due to its strong correlation with the forecasting error, as well as the marginal likelihood or evidence as a~\textbf{selection} strategy for question one.
Therefore, we replace the last layer of a neural network with a~\ac{blr}, as proposed in~\cite{You2021LogMe} for computer vision tasks. 
Second, we propose to utilize the~\ac{blr} as a model to~\textit{adapt} a source model to the target and answer question two. 
To ensure that we find the best adaption strategy, we \textit{directly} apply a source model on the target and consider the state-of-the-art such as weight decay as well as Bayesian tuning~\cite{You2021LogMe}. 
Considering the two selection strategies, we evaluate $18$ combinations making it the most extensive evaluation for~\ac{tl} in renewable power forecasts.
Third, due to the~\ac{blr} as the output layer, we propose~\textbf{combining} multiple source models through~\ac{bma} to answer question three. 
Finally, we propose the~\ac{csge} as ensemble technique for~\ac{itl}.
% \begin{enumerate}
%     \item We propose the~\ac{nrmse}, due to its strong correlation with the forecasting error, as well as the marginal likelihood or evidence as a~\textit{selection} strategy for question one, where we replace the last layer of a neural network by a~\ac{blr}, as proposed in~\cite{You2021LogMe} for computer vision tasks. 
%     \item We propose to utilize the~\ac{blr} as a model to~\textit{adapt} a source model to the target and answer question two. To ensure that we find the best adaption strategy, we \textit{directly} apply a source model on the target and consider the state-of-the-art such as weight decay as well as Bayesian tuning~\cite{You2021LogMe}. Thereby, considering the two selection strategies, we evaluate $18$ combinations making it the most extensive evaluation for~\ac{tl} in renewable power forecasts.
%     \item Due to the~\ac{blr} as the output layer, we propose~\textit{combining} multiple source models through~\ac{bma} to answer question three. Finally, we propose the~\ac{csge} as ensemble technique for~\ac{itl}.
% \end{enumerate}
The source code is open accessible\footnote{\url{https://github.com/scribbler00/DEELEA}, accessed 2022-07-15}.

The remainder of this article is structured as follows. 
~\SEC{sec_itl_selection_related_work} describes related work. 
The following~~\SEC{sec_itl_selection_method} introduces relevant definitions and details the proposed approach. 
We describe the datasets and discuss the experiment's most essential findings in~\SEC{sec_itl_selection_experiment}. 
In the final~\SEC{sec_itl_selection_conclusion}, we summarize our work and provide insights for future work.
% \todobox{The paper's signiﬁcance may be improved by discussing more the practical application of the model. Maybe
% provides a ﬂowchart that the practitioners can follow in case they want to use the same strategy outlined in the
% paper.}
\listofsymbols

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/method.tex <==
% TODO THESIS
\section{Proposed Methods}
\label{sec_itl_selection_method}
The following sections define the proposed model selection, model adaptation, and model combination strategies. 
Beforehand we introduce the~\ac{blr} as it is the basic model for one selection and one adaption strategy.
% We first summarize~\ac{blr} to calculate the evidence for model selection and define the~\ac{belm}.
% Afterward, we formalize the concept of model selection in~\ac{itl}, briefly summarize relevant adaptation strategies, and introduce~\ac{bma} and the~\ac{csge}.

\input{sections/inductive_transfer_learning/selection_and_ensembles/method_bayesian_linear_regression}
\input{sections/inductive_transfer_learning/selection_and_ensembles/method_model_selection}
\input{sections/inductive_transfer_learning/selection_and_ensembles/method_model_adaption}

\subsection{Model Combination for Inductive Transfer Learning}\label{sec_method_model_combination}
\input{sections/inductive_transfer_learning/selection_and_ensembles/method_bayesian_model_averaging}
\input{sections/inductive_transfer_learning/selection_and_ensembles/method_csge}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/method_bayesian_linear_regression.tex <==
\subsection{Bayesian Linear Regression}
% \label{sec_bayesian_linear_regression}
The following definitions of a~\ac{blr} makes use of the introductions in~\cite{Bishop2006} and~\cite{deisenroth2020mathematics}.
In contrast to a deterministic perspective to learn the model weights of a linear regression model, a Bayesian approach gives additional insights through the posterior, especially when there is insufficient data~\cite{Bishop2006} as for~\ac{tl}.
It helps in measuring task similarity for model selection and allows assessing the quality of the model in terms of its uncertainty, as proposed in~\cite{You2021LogMe}.
We propose to utilize it also for an adaptation for renewable forecasts.
We achieve this by replacing the final layer of a neural network with a~\ac{blr}, training it with the target data, and making predictions for the target afterward.
This approach additionally allows combining models through~\ac{bma}, see~\SEC{sec_method_model_combination}.
Finally, we can utilize it to learn a~\ac{belm}.

Therefore, let us assume that the following equation details the posterior distribution of such a linear model:
\begin{equation}
    \underbrace{p(\parametersLinModel|\setInputFeatures, \setOutputFeatures)}_{\text{posterior}} = \frac{\overbrace{p(Y|X, \parametersLinModel)}^{\text{likelihood}}\overbrace{p(\parametersLinModel}^{\text{prior}})}{\underbrace{p(\setOutputFeatures|\setInputFeatures)}_{\text{marginal likelihood}}},
\end{equation}
where $\setInputFeatures = \{\inputFeatureVector_n\}_{n=1}^{n=\nSamples}$ and $\setOutputFeatures=\{\outputFeatureVector_n\}_{n=1}^{n=\nSamples}$ are the sets of observed input and response values with $\nSamples \in \naturalNumberPos$ samples from a training dataset.
In this setting, a single feature vector $\inputFeatureVector_n \in \realNumber^\dimFeature$ has $\dimFeature \in \naturalNumberPos$ features and $\outputFeatureVector_n$ is of size $\realNumber$.
Then the likelihood $p(\setOutputFeatures|\setInputFeatures, \parametersLinModel)$ describes how well $\setInputFeatures$ 
and the weights $\parametersLinModel\in \realNumber^D$ describe the response values.
Through the prior, we encode our initial beliefs about the model weights.
The marginal likelihood normalizes the posterior.
Finally, after observing training data, the posterior encodes what we know about the target.

To calculate the distributions of the posterior of a linear regression model consider that we have a prior over the weights $\parametersLinModel$ with $p(\parametersLinModel|\alpha) = \normalDist(\parametersLinModel| 0, \alpha^{-1}\mathbf{I})$,
% \begin{equation}
%     p(\boldsymbol{\theta}|\alpha) = \normalDist(\boldsymbol{\theta}| 0, \alpha^{-1}\mathbf{I}),
% \end{equation}
where $\alpha \in \realNumberNonNeg$ is the precision of the zero mean isotropic Gaussian distribution.
Note, choosing an isotropic Gaussian distribution for the prior allows deriving a closed form solution that reduces computational effort for calculating the mean and covariance matrix, as detailed in the following.

Now consider that we have a target $\outputFeatures$ of size $1 \times N$ and $\inputFeatures$ is the $N \times \dimFeature$ design matrix, where each row corresponds to the $n$-th observation.
For multivariate problems, we can train one model per response.
% \todobox{eigentlich ist X immer irgendwie transformiert, es ist niemals direkt die wettervorhersage, sollte auch in der intro angepasst werden???!!!}
% Within this article $\inputFeatures$$ can be one of three things. First, it can be weather predictions such as wind or radiation from an~\ac{nwp}. Second, it can be features extracted from an neural network from the second last layer. Third, it can be random features from an BELM.
In our case, $\inputFeatures$ are either weather predictions from an~\ac{nwp} such as wind speed or radiation, random features from an~\ac{belm}, or features extracted from a neural network at the second last layer.
In the latter two cases the weather predictions are transformed through the neural network or the~\ac{belm}.
% Here, weather predictions such as wind or radiation from an~\ac{nwp}, from a neural network, or random features from a~\ac{belm}.
% Assuming that the weather features are given by $\hat{\inputFeatures}$, then $\inputFeatures$ of the~\ac{belm} is:
% \begin{equation*}
%     \inputFeatures = f(\hat{\inputFeatures}\mathbf{Q}),
% \end{equation*}
% where $f$ is a non-linear activation function and $\mathbf{Q}$ is a matrix of size $D\times C$, where $C \in \naturalNumberPos$ are the number of hidden neurons of the~\ac{belm} and $D$ is the number of features from the~\ac{nwp}.
% In contrast to an~\acp{mlp}, $\mathbf{Q}$ is not trained for~\acp{belm}. Instead, it is, e.g., sampled from a Gaussian distribution.

Finally, the posterior distribution is given by $\outputFeatures$, $\inputFeatures$, and the noise precision parameter $\beta \in \realNumberNonNeg$ through $p(\parametersLinModel| \inputFeatures, \outputFeatures) = \normalDist(\parametersLinModel | \mathbf{m}_N ,\precisionMatrix_N)$, where
% \begin{equation}
%     p(\boldsymbol{\theta}| \inputFeatures, \outputFeatures) = \normalDist(\boldsymbol{\theta} | \mathbf{m}_N ,\precisionMatrix_N),
% \end{equation}
% where $\mathbf{m}_N = \beta \precisionMatrix_N X^T \outputFeatures$ and $\precisionMatrix_N^{-1} = \alpha\mathbf{I} + \beta \inputFeatures^T\inputFeatures$.
\begin{equation}\label{eq_blr_online_update_mean}
    \mathbf{m}_N = \beta \precisionMatrix_N \inputFeatures^T \outputFeatures\text{~and~}\precisionMatrix_N^{-1} = \alpha\mathbf{I} + \beta \inputFeatures^T\inputFeatures.
\end{equation}
% \begin{equation}\label{eq_blr_online_update_precision}
%     \precisionMatrix_N^{-1} = \alpha\mathbf{I} + \beta \inputFeatures^T\inputFeatures.
% \end{equation}
In this setting, $\nSamples$ indicates the number of training samples used to update our prior beliefs of the model weights.
In most cases, we are interested in predicting an unknown response $\outputFeatures_{*}$ based on input $\inputFeatures_{*}$ from a (test) dataset not seen during the training of the model.
Therefore, the predictive posterior is defined by:
\begin{align}\label{eq_lin_predictive_posterior}
    p(\inputFeatures_{*}|\outputFeatures, \alpha, \beta) & =  
    \int p(\inputFeatures_{*}|\outputFeatures, \parametersLinModel) p(\parametersLinModel|\inputFeatures, \outputFeatures) \text{d}\parametersLinModel \nonumber \\                                                 &=\normalDist(y_{*}|\inputFeatures_{*} \mathbf{m}_N, \boldsymbol{\sigma}_N^2(\inputFeatures_{*})),
\end{align}
where $\outputFeatures$ and $\inputFeatures$ are from the training set and the posterior variance is given by
\begin{equation}
    \boldsymbol{\sigma}^2_N(\inputFeatures_{*}) = \beta^{-1} + \inputFeatures^T_{*} \precisionMatrix_N \inputFeatures_{*}.
\end{equation}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/method_bayesian_model_averaging.tex <==
% \subsection{Bayesian Model Averaging for Model Combination}
% \label{sec_method_bma}
We discussed the model selection and adaptation strategies for a single source model for a target.
However, a single model might be prone to overfitting with limited data.
Combining source models through an ensemble reduces this risk.

\subsubsection{Bayesian Model Averaging} 
We extend the concept of~\cite{You2021LogMe} so that instead of choosing a single model based on the evidence, we combine models adapted through~\ac{blr} by~\ac{bma}.
\Ac{bma} is theoretically appealing as it considers the predictive posterior~\cite{Hoeting1999} and therefore considers the uncertainty of a model through
% https://projecteuclid.org/journals/statistical-science/volume-14/issue-4/Bayesian-model-averaging--a-tutorial-with-comments-by-M/10.1214/ss/1009212519.full
\begin{equation}\label{eq_bayesian_model_averaging}
    p(\outputFeatures_{T*}|\outputFeatures_T) = \sum_{i=1}^{i=M}p(\outputFeatures_{T*}|\outputFeatures_T, \parametersLinModel_{M_i}) p(\parametersLinModel_{M_i}|\outputFeatures_T).
\end{equation}
The prior probability $p(\parametersLinModel_{M_i}|\outputFeatures_T)$ encodes our prior belief that a model $M_i$ is more likely to another one for the target data set.
For simplicity, we consider an equal prior for all source models.
Note that we have omitted the input here to simplify notations.
% This prior can be either selected or can be calculated.
% In case of a calculation, the model posterior can be approximated through the empirical Bayes and therefore the marginal likelihood,~\todobox{see page 175 in murphy}.
% For example, by the posterior of the training data.
% \todobox{seite 158 und 583 murphy}
% through the marginal likelihood with~\EQ{eq_marginal_likelihood}\todobox{seite 138 eq 4.225 in bishop}.
$p(\outputFeatures_{T*}|\outputFeatures_T, \parametersLinModel_{M_i})$ is the predictive posterior of a model $M_i$ given by~\EQ{eq_lin_predictive_posterior}, where, e.g, the model results from the proposed~\textit{direct linear} adaptation strategy.
% \todobox{In the following, we give two examples of Bayesian model averaging}.
% The first example uses the log evidence of a model to calculate a~\ac{bma} model.
% However, this approach is applicable only if both models have the same input face.
% This holds as the marginal likelihood is only aware of differences between models in the hyperparameter of the model.
% At the same it can be argued that this is an advantage as it also considers the model complexity.
% Therefore, it favors simpler models with fewer weights to tune.

% The second approach uses the predictive uncertainty to calculate the weighting scheme for the ensemble.
% This approach has the disadvantage of not considering the differences in hyperparameter.
% However, it is also applicable when two models have different input regions.

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/method_csge.tex <==

\subsubsection{Coopetitive Soft Gating Ensemble:} We also propose to utilize the~\ac{csge} for model combination in the context of~\ac{itl}.
The~\ac{csge} was initially introduced for renewable power forecast in~\cite{GS18}.
The idea of the CSGE is to link the weights to the ensemble members' performance, i.e., good source models are weighted stronger than weaker ones.
The~\ac{csge} characterizes the overall weight of a source model using three aspects:
\begin{itemize}
    \item The \textit{global weight} is defined by how well a source model performs with the available training data on the target task.
    \item The \textit{local weight} is defined by how well a source model performs on the target tasks for different areas in the feature space. For example, in the case of wind, one model might perform well for low wind speeds, while another source model might perform well for larger wind speeds on the target.
    \item The \textit{forecast horizon-dependent weight} is defined by how well a source model performs for different lead times on the target task. Here, between $24$ and $48$ hours into the future.
\end{itemize}
\begin{figure*}[tb]
    \centering
    \input{sections/inductive_transfer_learning/selection_and_ensembles/figures/overview_csge}
    \caption{The architecture of the CSGE. The source models' predictions $\outputPredictionVector^{(\indexSourceModel)}_{t + k | t}$ for the input $\inputFeatureVector$ are passed to the CSGE. The ensemble member's weights are given by aggregating the respective global-and local- and forecast horizon-dependent weights. The weights are normalized. The source models' predictions are weighted and aggregated in the final step.}
  
    \label{fig:coop_int_fusion:csge_overview_graphic}
\end{figure*}

Fig.~\ref{fig:coop_int_fusion:csge_overview_graphic} provides an overview of the~\ac{csge}.
The CSGE includes $\numberSourceModels$ ensemble members, with $\indexSourceModel \in \{1, \ldots, \numberSourceModels\}$.
Each of these ensemble members is a source model with a predictive function $f_\indexSourceModel$. %TODO THESIS according to~\DEF{def_task} and~\ref{def_itl}.
Each source model forecasts an univariate estimate $\hat{y}^{(\indexSourceModel)}_{t + k | t} \in \mathbb{R}$ for the input $\inputFeatureVector_{t + k | t} \in \mathbb{R}^{\dimFeature}$ of a target task $\indexTargetTask$, we omit the subscript $\indexTargetTask$ for reasons of clarity and comprehensibility.
Let $\dimFeature$ be the dimension of the input feature vector $\inputFeatureVector$.
Then, $k$ denotes the forecast horizon, denoted by the subscript, for the forecast origin $t$.
For each prediction of each source model, we compute an aggregated weight $\csgeWeightNormalized^{(\indexSourceModel)}_{t + k | t}$.

The weight incorporating the global $w_g$, local $w_l$, and forecast horizon-dependent weight $w_h$ for a single source model and lead time is given by
\begin{align}
    \label{eq:coop_int_fusion:csge:overallweights}
    \csgeWeightUnnormalized^{(\indexSourceModel)}_{t + k | t} = \csgeWeightNormalized^{(\indexSourceModel)}_g \cdot \csgeWeightNormalized^{(\indexSourceModel,t)}_l \cdot \csgeWeightNormalized^{(\indexSourceModel,k)}_{h},
\end{align}
where $\csgeWeightUnnormalized^{(\indexSourceModel)}_{t + k | t}$ is normalized to sum up to one to calculate $\csgeWeightNormalized^{(\indexSourceModel)}_{t + k | t}$.

To calculate the weights $\csgeWeightNormalized^{(\indexSourceModel)}_{t + k | t}$, we utilize the definition of the inverse similarity measurement $\similarityMeasure^{-1}$ from~\SEC{sec_model_selection_definition} and the coopetitive soft gating principle from~\EQ{eq_soft_gating}.
\begin{align}\label{eq_soft_gating}
    \varsigma^{'}_\eta(\mathbf{\Phi}, \phi) = \frac{\sum_{j=1}^{J} \mathbf{\Phi}_j}{\phi^{\eta} + \epsilon}
\end{align}
By calculating the weighting through the inverse $\similarityMeasure^{-1}$, here the~\ac{nrmse}, we estimate how well a source model performs on the target.
Let us assume that $\mathbf{\Phi} \in \realNumber^{J}$ contains all $J \in \naturalNumberPos$ estimates based on the~\ac{nrmse} and $\phi \in \mathbf{\Phi}$.
Then, $\eta \geq 0$ depicts the amount of exponential weighting and the small constant $\epsilon > 0$ avoids division by zero.
For greater $\eta$, the \ac{csge} tends to work as a gating ensemble, thereby considering only a few source models.
For smaller $\eta$ result in a weighting ensemble.
After calculating all weights from $\mathbf{\Phi}$ through~\EQ{eq_soft_gating}, we normalize the results to sum up to one estimating the final weights $\csgeWeightNormalized^{(\indexSourceModel)}_{t + k | t}$.
This approach is repeated for each of the three weighting aspects as detailed in~\cite{GS18} and~\ref{sec_appendix_model_selection_method}.


==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/method_model_adaption.tex <==
\subsection{Adaptation Strategies for Inductive Transfer Learning}
\label{sec_itl_selection_method_adaption}
\TBL{tbl_model_selection_overview} overviews all $18$ combinations of models and adaptation strategies.
As a simple~\ac{tl} model, we consider an \textit{online} update of the posterior of the~\ac{belm}.
Therefore, the posterior from a source model acts as a prior for the target.
Additionally, we evaluate \textit{directly} applying a selected source model on the target without any adaptation of a source model's parameter.

We also consider two standard fine-tuning methods from the field of computer vision.
The first one is \textit{weight decay} which penalizes the deviation of weights from zero and \textit{weight decay source} which penalizes a deviation from the source model's weights.
Additionally, we examine \textit{Bayesian tunning} as introduced in~\cite{You2021Hub}.


% \end{enumerate}
\begin{table*}[tb]
    % \footnotesize
    \centering
    \caption{Overview of different combinations for models, selections, and adaptations. RM abbreviates the RMSE selection strategy, EV the selection through evidence, DI stands for directly applying the model, WD for fine-tuning through weight decay regarding the origin, WDS for a fine-tuning through weight decay regarding the source parameters, BT for fine-tuning with Bayesian tuning.}\label{tbl_model_selection_overview}
    \begin{tabular}{l|l|l|l}
        % \hline
        \textbf{Model}   & \textbf{Selection} & \textbf{Adaptation}            & \textbf{Abbreviation}  \\
        \textbf{Type}    & \textbf{Strategy}  & \textbf{Strategy}            &               \\
        % \hline
        \hline
        MLP/TCN & RMSE~[ours]      & direct~[ours]             & MLP-/TCN-RM-DI   \\
        % \hline
        MLP/TCN & RMSE~[ours]      & weight decay~\cite{Li2020}        & MLP-/TCN-RM-WD   \\
        % \hline
        MLP/TCN & RMSE~[ours]      & weight decay source~\cite{Li2018} & MLP-/TCN-RM-WDS  \\
        % \hline
        MLP/TCN & EVIDENCE~\cite{You2021Hub}  & direct~[ours]             & MLP-/TCN-EV-DI   \\
        % \hline
        MLP/TCN & EVIDENCE~\cite{You2021Hub}  & direct linear [ours]      & MLP-/TCN-EV-DILI \\
        % \hline
        MLP/TCN & EVIDENCE~\cite{You2021Hub}  & weight decay~\cite{Li2020}         & MLP-/TCN-EV-WD   \\
        % \hline
        MLP/TCN & EVIDENCE~\cite{You2021Hub}  & weight decay source~\cite{Li2018} & MLP-/TCN-EV-WDS  \\
        % \hline
        MLP/TCN & EVIDENCE~\cite{You2021Hub}  & Bayesian tuning~\cite{You2021Hub}     & MLP-/TCN-EV-BT   \\
        % \hline
        BELM     & RMSE~[ours]      & Online~[ours]            & BELM-RM       \\
        % \hline
        BELM     & EVIDENCE~\cite{You2021Hub}  & Online~[ours]            & BELM-EV       \\
        % \hline
    \end{tabular}
\end{table*}


The three latter adaption strategies can be considered as a type of regularization.
In general, this means that we add an additional penalty term $L_{pen}$ to the loss function $L_{task}$ of a task through
\begin{equation}
    L = L_{task} + \lambda \cdot L_{pen}, 
\end{equation}
where $\lambda \in \mathcal{R}$ is a hyper-parameter for the amount of regularization that is typically selected by hyper-parameter optimization.
$L_{task}$ is given by
\begin{equation}
    L_{task} = \frac{1}{\nSamples}\sum^\nSamples_{\indexSamples=1}{l(f(\inputFeatureVector_\indexSamples, \boldsymbol{\theta}),\outputFeatureVector_\indexSamples)},
\end{equation}
where $\parametersLinModel \in \realNumber^p$ and $p\in\naturalNumberPos$ is a vector of the parameters we update, $\inputFeatureVector_\indexSamples$ is the $\indexSamples$-th input vector with $\indexSamples \in \nSamples$ and $\nSamples\in\naturalNumberPos$, and $\outputFeatureVector_\indexSamples$ is the respective response.
For simplicity, we consider a uni-variate response here.
For weight decay (WD) with respect to the origin~\cite{Li2020}, $L_{pen}$ is then given by
\begin{equation}
    L_{WD} = \frac{1}{2}||\boldsymbol{\theta}||^2_2
\end{equation}
To penalizes a deviation from the source model, \cite{Li2018} proposes a weight decay w.r.t. to source weights (WDS) given by
\begin{equation}
    L_{WDS}  = \frac{1}{2}||\boldsymbol{\theta}-\boldsymbol{\theta}^0||^2_2,
\end{equation}
where $\parametersLinModel^0 \in \realNumber^p$ is the vector of parameters from the source model before fine-tunning.
Finally, in Bayesian tunning $L_{pen}$ is given by~\cite{You2021Hub}:
\begin{equation}
    L_{Bayesian} = \frac{1}{\nSamples}\sum^{\nSamples}_{\indexSamples=1}{\frac{1}{K}\sum^{K}_{k=1}}{(\frac{1}{M}\sum^{M}_{\indexSourceModel=1}{\inputFeatureVector_{\indexSourceModel,\indexSamples}^T\parametersLinModel_{\indexSourceModel,k}-\inputFeatureVector_{t,\indexSamples}^T\parametersLinModel_{t,k}})^2},
\end{equation}
where $\indexSamples \in \nSamples$ is the $\indexSamples$-th data sample, $\indexSourceModel$ is the $\indexSourceModel$-th source model adapted with~\ac{blr}, $k$ is the $k$-th dimension of the response for example for different forecast horizons.
$\inputFeatureVector_{\indexSourceModel,k}$ are features extracted from the $\indexSourceModel$-th source model, $\inputFeatureVector_{t,\indexSamples}$ are the respective features extracted from the target model $t$.
$\parametersLinModel_{k,c}$ and $\parametersLinModel_{t,c}$ are the mean vectors calculated by the~\ac{blr}.

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/method_model_selection.tex <==
\subsection{Model Selection for Inductive Transfer Learning}\label{sec_model_selection_definition}

Measuring task similarity between a target task and multiple source tasks is a critical challenge in~\ac{itl}~\cite{You2021LogMe} as it allows selecting an appropriate source task for knowledge transfer.
Ideally, a valid model selection avoids negative transfer, so utilizing knowledge from the source model has a minor error than training a target model from scratch.

\begin{figure}
    \centering
    \input{sections/inductive_transfer_learning/selection_and_ensembles/figures/bayesian_model_selection}
    \caption{Bayesian model selection adapted from~\cite{deisenroth2020mathematics}.}
    \label{fig_bayesian_model_selection}
\end{figure}
% \subsubsection{}
Before we formalize the concept of model selection in the context of~\ac{tl} we will provide an intuition behind (Bayesian) model selection in a broader sense.
In~\cite{Bishop2006}, it is argued that a model selection (outside the context of~\ac{tl}) approach should find a trade-off between model complexity and the fit for the data.
This trade-off is visualized from a Bayesian perspective in~\FIG{fig_bayesian_model_selection}.
On the horizontal axis, the space of all possible datasets is given.
The evidence of a model for a given dataset $\mathcal{D}_T$ is given on the vertical axis.
In this case, consider that model $M_2$ is a larger model with more parameters than model $M_1$ and, therefore, can express a larger number of datasets.
We can see that with the model evidence $p(\mathcal{D}|M_\indexSourceModel)$ we would favor the simpler model for dataset $\mathcal{D}_T$ through the Bayesian perspective.
The concept that a Bayesian perspective on model selection favors the simpler model is also known as \textit{Occam's razor}.

The general concept of model selection is also valid in the context of~\ac{tl}.
We aim to find a source model, from $m \in \{1,\ldots,M\}$ source models with $M \in \mathbb{N}_{>1}$, that explains the limited target data $T$ best.
Consider two tasks $\task_1 = \{ \outputFeatureSpace,~P_1(\setOutputFeatures_1 \mid \setInputFeatures_1)\}$ and $\task_2 = \{ \outputFeatureSpace,~P_2(\setOutputFeatures_2 \mid \setInputFeatures_2)\}$, where the tasks $\task_1,\task_2 \in \allTasks$ and $\allTasks$ is the set of all possible tasks.
The sets $\setOutputFeatures_m$ and $\setInputFeatures_m$ are from the response space $\outputFeatureSpace$ and feature space $\inputFeatureSpace$.
By defining a similarity measure $\similarityMeasure$ with $\similarityMeasure \colon \allTasks \times \allTasks \to \realNumberPos$, the mapping into a scalar allows making quantitative statements.
For instance, given two source tasks $\task_1, \task_2$ and a target task $\task_T$ if $\similarityMeasure\big(\task_1,\task_T\big) > \similarityMeasure\big(\task_2,\task_T\big)$ then $\task_1$ is more similar to the target $\task_T$ compared to $\task_2$, which means, that a high value implicates a high similarity.
Respectively, we define dissimilarity by the inverse of a similarity measure.

Now the question arises what (similarity) measure and what kind of data should be considered to select a source model from a model hub for a specific target.
One choice would be to measure similarity solely based on the input feature space.
However, the input feature space contains limited information on the expected power generation, the response variable, in renewable power generation.
For example, different amounts of energy will be produced with the same radiation for different solar modules.
Consequently, we need to take the response variable into account.

% In the following, we extend the concept of a task and domain, see~\DEF{def_task} and~\ref{def_domain}, to measure similarities between tasks.
% Measuring task similarity, for model selection, between a target task and multiple source tasks is a critical challenge in~\ac{itl}~\cite{You2021LogMe}.
% It allows selecting an appropriate source task for knowledge transfer.
% A valid model selection avoids negative transfer so that utilizing knowledge from the source model has a minor error than training a target model from scratch.
% We aim to find a source model, from $m \in \{1,\ldots,M\}$ source models with $M \in \mathbb{N}_{>1}$, that explains the limited target data $T$ best.
% Consider two tasks $\task_1 = \{ \outputFeatureSpace,~P_1(\setOutputFeatures_1 \mid \setInputFeatures_1)\}$ and $\task_2 = \{ \outputFeatureSpace,~P_2(\setOutputFeatures_2 \mid \setInputFeatures_2)\}$, where the tasks $\task_1,\task_2 \in \allTasks$ and $\allTasks$ is the set of all possible tasks.
% The sets $\setOutputFeatures_m$ and $\setInputFeatures_m$ are from the response space $\outputFeatureSpace$ and feature space $\inputFeatureSpace$.
% By defining a similarity measure $\similarityMeasure$ with $\similarityMeasure \colon \allTasks \times \allTasks \to \realNumberPos$, the mapping into a scalar allows making quantitative statements.
% For instance, given two source tasks $\task_1, \task_2$ and a target task $\task_T$ if $\similarityMeasure\big(\task_1,\task_T\big) > \similarityMeasure\big(\task_2,\task_T\big)$ then $\task_1$ is more similar to the target $\task_T$ compared to $\task_2$, which means, that a high value implicates a high similarity.
% Respectively, we define dissimilarity by the inverse of a similarity measure.

\subsubsection{Evidence or Marginal Likelihood:} The authors of~\cite{You2021LogMe} utilize the marginal likelihood or evidence as a similarity measure $\similarityMeasure$.
For that purpose, the final layer of a (source) neural network $\task_m$ is replaced by a~\ac{blr}, where the priors $\alpha$ and $\beta$ of this model are optimized through empirical Bayes~\cite{You2021Hub,Bishop2006} on limited target data.
In this way, the source model acts as a feature extractor.
% The linear model is trained with the limited training data from the target and the extracted features from the source model are, therefore, transformed through the linear regression model to predict the expected power.
% Based on the trained linear regression model we can calculate the marginal likelihood from the available target training data through
The marginal likelihood is then given by
\begin{align}\label{eq_marginal_likelihood}
   \similarityMeasure(\task_T,\task_m) &=  \ln p(\outputFeatures|\alpha,\beta)  \nonumber \\
        &= \frac{D}{2}\ln \alpha + \frac{N}{2} \ln \beta - E(\mathbf{m}_N) - \frac{1}{2}\ln{|\mathbf{S}^{-1}_N| - \frac{N}{2}\ln{2\pi}},
\end{align}
where $D$ is the number of features, e. g., defined by the dimension of the second last layer of the neural network $m$ with $N$ samples and $E(\mathbf{m}_n) = \frac{\beta}{2} \cdot ||\outputFeatures - \inputFeatures \mathbf{m}_n|| + \frac{\alpha}{2} \mathbf{m}_n^T \mathbf{m}_n$. 
This way, we consider features extracted from the source neural network of task $\task_m$ and the response feature from the target $\task_T$.
If we do this for each source model $m$, we can calculate the marginal likelihood of each source model on the target to calculate $\similarityMeasure(\task_m, \task_T)$.
We then select the model with the most extensive evidence as the appropriate source model.
We repeat this for each dimension for multivariate problems and average the results~\cite{You2021LogMe}.

While this approach is theoretically appealing and generalizes for a broad number of problems, it has one drawback in the context of \ac{itl}: It is not considering already learned weights from the final layer of a model.
This consideration is essential, as we often do not need to remove the final layer to assure compatibility between a source and a target task in renewable energies.
At the same time, a pre-trained layer is usually beneficial in contrast to a randomly initialized layer.

\subsubsection{Normalized Root Mean-squared Error:}
% Neglecting the final layer can be circumvented through the~\ac{nrmse} given by
Respectively, we propose to directly measure the similarity through the~\ac{nrmse} based on the pre-trained layer of a source model by
\begin{equation}\label{eq_nrmse}
    \similarityMeasure(\task_T,\task_m)^{-1} = \text{nRMSE} = \sqrt{\frac{1}{N}\sum_{i=1}^{i=N}{(y_i^{(T)}-\hat{y}_i^{(m)})^2}},
\end{equation}
where $y_i^{(T)}$ is the $i$-th normalized response from the target and $\hat{y}_i^{(m)}$ is the prediction from source model $m$ on the target.
Note that in the context of renewable power forecasts, we normalize the response $y_i$ by the nominal power to assure comparability of the error for different parks.
We can directly measure how well a source model performs on the available target data to measure the similarity $\similarityMeasure(\task_m, \task_T)$.
Consequently, we can select the source model with a lower~\ac{nrmse} on, e.g., a validation error from the target data.
% During initial experiments, we found that only utilizing a suitable selection strategy is insufficient to capture the problem of~\ac{itl} with limited data in the domain of power forecasts.
% Besides the selection strategy, the test error on the target with limited data also depends on the adaptation strategy.
% Adaptation strategy refers here to the applied~\textit{method} of knowledge transfer from the source to the target.
% In the naive approach, we can utilize a source model directly on the target for homogenous~\ac{itl}.
% In the following, we refer to this approach as \textit{direct} adaptation strategy.
% Another approach is the utilization of the Bayesian linear regression that replaces the final layer of the source model and is trained with features extracted from the source model and trained with response variables from the target referred to as \textit{direct linear} adaptation.
% \todobox{We can extend this approach to not only remove the last layer, but also the second last layer, and then we can select the model with the highest evidence, and this one is used to forecast the target, referred to as \textit{direct linear auto} for the automatic selection for the removal of the number of layers of the neural network.}
% A more well-known approach is to train a source model with target data and limit the effects of catastrophic forgetting through penalization terms.
% This penalized term is most often \textit{weight decay}.
% More recently, \textit{Bayesian tunning} was suggested as adaptation strategy~\CN{LOGME2}
% ($E(\mathbf{m}_n)$ is the same as the negative posterior of the mean vector)
% The marginal likelihood can also be understand as the expected likelihood under a given prior, i. e., $\mathbb{E}_{\mathbf{W}}[p(\mathcal({Y}|\mathcal{X},\mathbf{W}]$.
% \todobox{have an example how this can be used for model selection}
% \subsubsection{Probablistic Similarity Measures}
% \subsubsubsection{Log-likelihood}: The log-likelihood is given by
% \todobox{in formula: LL of what?}
% \begin{equation}
%     \text{LL} = -\frac{N}{2} \cdot \ln{2\cdot\pi}-\frac{N}{2} \cdot \ln{\underbrace{\sigma^2}_{\text{MSE}}}-\frac{1}{2\cdot\sigma^2} \underbrace{\sum_{i=0}^{i=N}{(y_i-\hat{y})^2}}_{\text{RSS}}
% \end{equation}
% assuming an isotropic Gaussian of the target $y$ with
% \begin{equation}
%     p(y|\mathbf{X},\mathbf{W}) = \mathcal{N}(y|XW, \beta^{-1}\cdot I)
% \end{equation}
% where the $\beta$ is the precision (inverse variance) with $\frac{1}{\beta}=\sigma^2=MSE$.
% \subsubsubsection{Akaike and Bayesian information criterion}:
% Often, we don't have access to a complete probabilistic perspective of a model.
% To compensate for the full Bayesian treatment a number of model selection heuristics such as the \ac{aic} have been developed given by
% \todobox{make relation to model comparision}
% \todobox{highlight differences between the two}
% \todobox{motivate how BIC can be used to select the number of layers to transfer in an MLP...}
% \begin{equation}
%     \log (p|\mathbf{X}|\mathbf{W})  - M,
% \end{equation}
% where $M$ is the number of parameters.
% Essentially, the~\ac{aic} measure the relative information lost, with respect to the number of parameters, by an optimized model.
% Similar the~\ac{bic} can be used to measure similarity or express the goodness of fit of a model:
% \begin{equation}
%     \log p(\mathbf{x}) = \log \int p(\mathbf{x}|\mathbf{W}) p(\mathbf{W}) \approx \log (p(\mathbf{X|\mathbf{W}})) - \frac{1}{2} M \log N,
% \end{equation}
% where N is the number of samples.\todobox{M to the power of i, for the number of layers?}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/selection_and_ensembles.tex <==
\input{sections/inductive_transfer_learning/selection_and_ensembles/introduction}
\input{sections/inductive_transfer_learning/selection_and_ensembles/state_of_the_art}
\input{sections/inductive_transfer_learning/selection_and_ensembles/method}
\input{sections/inductive_transfer_learning/selection_and_ensembles/experiment}
\input{sections/inductive_transfer_learning/selection_and_ensembles/conclusion}

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/sections/inductive_transfer_learning/selection_and_ensembles/state_of_the_art.tex <==
% \subsection{Related work}
% TODO THESIS
\section{Related work}
\label{sec_itl_selection_related_work}
In the following section, we overview recent developments for~\ac{tl} and, more specifically for~\ac{itl} in computer vision that has been not considered for renewable power forecasts.
This review determines relevant techniques that we consider for renewable power forecasts.
Afterward, we summarize related work for~\ac{itl} on deterministic renewable power forecasts.

There are two crucial dimensions in~\ac{itl}.
The first is the model selection and the second is the adaptation strategy.
The authors of~\cite{You2021LogMe,You2021Hub} provide a study on selection strategies for the field of computer vision.
They utilize a~\ac{blr} replacing the final layer of a source model and train it through empirical Bayes, also referred to as evidence approximation, on the target data.
The authors repeat this approach for each available model from the model hub.
Finally, they determine the similarity through the evidence of a source model on the target.
% Compared to other selection strategies, this approach generalizes for regression, classification, and even multi-variate prediction problems.
As an adaptation strategy, they proposed Bayesian tuning, which regularizes the fine-tuning process by predictions from multiple sources.
% , adapted through the~\ac{blr}~\cite{You2021Hub}.
These proposed selections and adaptations need to be considered and extended for renewable energies.
For instance, we can directly forecast through the~\ac{blr} and compare it with fine-tuning of the final layer.
Often, the adaptation through fine-tuning is regularized by a weight decay regarding zero~\cite{Li2020}.
However, this regularizer does not consider parameters originating from the source model.
Therefore, in~\cite{Li2018} a deviation from a source model is penalized by weight decay considering the source model parameters.

Compared to research areas like computer vision, there is limited research on~\ac{itl} for renewable power forecasts, compare~\cite{Alkhayat2021}.
There has been some work to learn a transferable representation of the input utilizing autoencoders~\cite{Qureshi2019,Liu2021,Ju2020,Henze2020}.
While the principle approach of transferring an autoencoder for a target is combinable with our approach, we argue that considering the conditional distribution of the power forecast is more relevant for model selection and combination.
The data driven~\ac{tl} approaches presented in~\cite{Cao2018} and \cite{Cai2019} are outside the scope of this article.

Also, most of the current research on~\ac{tl} in renewable power forecasts focuses on meteorological measurements as input features, see \cite{Liu2021,Ju2020,Cao2018,Liu2022,Chen2020,Sheng2022,Yin2021,Khan2022,Almonacid2022,Yan2019}. 
These articles consider forecast horizons between ten seconds and two hours. 
At the same time, larger forecast horizons, such as day-ahead forecasts, are inherently more difficult as they utilize~\ac{nwp} as input features and forecast errors increase with an increasing forecast horizon~\cite{Jens2019}.

Most of the previously mentioned related work for~\ac{tl} in renewable energies is treating power forecast not as a time series approach.
Instead, the authors treat it as a regression.
At the same time, periodic influences from, e.g., the diurnal cycle, are well known.
Therefore, the authors of \cite{Zhou2020} consider recurrent networks and fine-tuning to achieve good results for an ultra-short-term forecast horizon of~\ac{pv}.
Additionally, the article \cite{Schreiber2021} considers time series methods in a~\ac{mtl} architecture.

The authors of~\cite{Ceci2017} achieve improvements in day-ahead~\ac{pv} forecasts through multi-target models.
The idea of model combination is similar to our ensemble approach.
However, the authors of this article do not evaluate it in the context of~\ac{itl}.
The study of~\cite{Shireen2018} proposes an \ac{mtl} strategy for Gaussian processes to forecast \ac{pv} targets.
By clustering wind parks, a weighting scheme provides predictions for a new park in~\cite{Tasnim2018}.
In this article, no actual historical power measurements are used for evaluation; instead, the authors used synthetic data.

A number of articles apply~\ac{mtl} architectures for~\ac{tl}~\cite{Schreiber2021,Vogt2019,Schreiber2020} in day-ahead forecasts.
The proposed task embedding in~\cite{Schreiber2021} and~\cite{Vogt2019} for~\acp{mlp} and~\acp{cnn}, encodes task-specific information through an embedding to learn latent similarities between tasks.
The article~\cite{Schreiber2021} is especially interesting as we have a similar experimental set-up.

However, the authors look at errors per season and results can be misleading as an~\ac{itl} approach should avoid catastrophic forgetting for all seasons.
Also,~\ac{mtl} architectures are due to their additional training complexity not common in the industry, e.g., due to data pre-processing and training complexity.
Therefore, for the extension of renewable energies making the best use of existing single-task models for~\ac{itl} is essential.

Furthermore, none of the related work studies different model selection and model adaptation strategies for neural network architectures.
While there has been some work on combining knowledge from multiple sites for~\ac{pv} through ensemble-like strategies, the studies are insufficient as they do not consider the amount of available data.
Also, the expected power is solely based on a characteristic curve, or authors consider solely~\ac{pv} or wind data.
We close these research gaps by providing an extensive study that overcomes those limitations for day-ahead forecasts.
% The article~\cite{Zang2020} provides a strategy for quantile regression for day-ahead solar power forecasts using~\acp{cnn} and fine-tuning.
% \begin{itemize}
%     \item most evaluations either wind or PV, but not both
%     \item much ultra-short stuff
%     \item
% \end{itemize}
% An extensive study on the influence of hyperparameters on the model adaptation is given in~\cite{Li2020}.

==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/setup.tex <==
% \newtheorem{definition}{Definition}

% \usepackage[pdftex]{graphicx}
% \usepackage{epstopdf}
\usepackage{microtype}
\usepackage[utf8]{inputenc}
\usepackage{booktabs}
\usepackage[shortcuts,acronym]{glossaries}
\usepackage{xcolor}
\usepackage{siunitx}
\usepackage[hyphens]{url}
% \usepackage{nameref}
% 
\usepackage[misc,geometry]{ifsym}

% \usepackage{times}
\usepackage[scaled]{helvet}
\usepackage{lscape}
\usepackage[hidelinks]{hyperref}
\usepackage{tikz}
% from csge paper
\usepackage{bm}
% \usepackage{subcaption}
\usepackage{diagbox}
\usepackage{siunitx}
% TODO THESIS
% \usepackage{fancyhdr}
\usepackage{amsfonts}

% for tikz plots
\usepackage{pgfplots}
\usetikzlibrary{calc}
\pgfplotsset{compat=1.8}
\usetikzlibrary{shapes,arrows}

\newcommand{\myline}[2]{
	\path(#1.east) --(#2.west)  coordinate[pos=0.4](mid);
	\draw[-latex] (#1.east) -| (mid) |- (#2.west);
}
\usepackage[caption=false]{subfig}
% ---
\sisetup{
	round-mode = places,
	round-precision = 3
}%
\definecolor{darkgreen}{RGB}{0,100,0}
\usepackage[final]{listofsymbols} % Symbolverzeichnis
%\usepackage[final]{listofsymbols} % Symbolverzeichnis
% \makeglossaries % generates the acronym list



==> Model Selection, Adaptation, and Combination for Deep Transfer Learning through Neural Networks in Wind and Solar Power Forecasts/splncs <==
%% BibTeX bibliography style `splncs03'
%%
%% BibTeX bibliography style for use with numbered references in
%% Springer Verlag's "Lecture Notes in Computer Science" series.
%% (See Springer's documentation for llncs.cls for
%% more details of the suggested reference format.)  Note that this
%% file will not work for author-year style citations.
%%
%% Use \documentclass{llncs} and \bibliographystyle{splncs03}, and cite
%% a reference with (e.g.) \cite{smith77} to get a "[1]" in the text.
%%
%% This file comes to you courtesy of Maurizio "Titto" Patrignani of
%% Dipartimento di Informatica e Automazione Universita' Roma Tre
%%
%% ================================================================================================
%% This was file `titto-lncs-02.bst' produced on Wed Apr 1, 2009
%% Edited by hand by titto based on `titto-lncs-01.bst' (see below)
%%
%% CHANGES (with respect to titto-lncs-01.bst):
%% - Removed the call to \urlprefix (thus no "URL" string is added to the output)
%% ================================================================================================
%% This was file `titto-lncs-01.bst' produced on Fri Aug 22, 2008
%% Edited by hand by titto based on `titto.bst' (see below)
%%
%% CHANGES (with respect to titto.bst):
%% - Removed the "capitalize" command for editors string "(eds.)" and "(ed.)"
%% - Introduced the functions titto.bbl.pages and titto.bbl.page for journal pages (without "pp.")
%% - Added a new.sentence command to separate with a dot booktitle and series in the inproceedings
%% - Commented all new.block commands before urls and notes (to separate them with a comma)
%% - Introduced the functions titto.bbl.volume for handling journal volumes (without "vol." label)
%% - Used for editors the same name conventions used for authors (see function format.in.ed.booktitle)
%% - Removed a \newblock to avoid long spaces between title and "In: ..."
%% - Added function titto.space.prefix to add a space instead of "~" after the (removed) "vol." label
%% - Added doi
%% ================================================================================================
%% This was file `titto.bst',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `vonx,nm-rvvc,yr-par,jttl-rm,volp-com,jwdpg,jwdvol,numser,ser-vol,jnm-x,btit-rm,bt-rm,edparxc,bkedcap,au-col,in-col,fin-bare,pp,ed,abr,mth-bare,xedn,jabr,and-com,and-com-ed,xand,url,url-blk,em-x,nfss,')
%% ----------------------------------------
%% *** Tentative .bst file for Springer LNCS ***
%%
%% Copyright 1994-2007 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2007/04/24 4.20 (PWD, AO, DPC)]
 %   For use with BibTeX version 0.99a or later
 %-------------------------------------------------------------------
 % This bibliography style file is intended for texts in ENGLISH
 % This is a numerical citation style, and as such is standard LaTeX.
 % It requires no extra package to interface to the main text.
 % The form of the \bibitem entries is
 %   \bibitem{key}...
 % Usage of \cite is as follows:
 %   \cite{key} ==>>          [#]
 %   \cite[chap. 2]{key} ==>> [#, chap. 2]
 % where # is a number determined by the ordering in the reference list.
 % The order in the reference list is alphabetical by authors.
 %---------------------------------------------------------------------

ENTRY
  { address
    author
    booktitle
    chapter
    doi
    edition
    editor
    eid
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    url
    volume
    year
  }
  {}
  { label }
INTEGERS { output.state before.all mid.sentence after.sentence after.block }
FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}
STRINGS { s t}
FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
        { add.period$ write$
%          newline$
%          "\newblock " write$  % removed for titto-lncs-01
          " " write$            % to avoid long spaces between title and "In: ..."
        }
        { output.state before.all =
            'write$
            { add.period$ " " * write$ }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}
FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}
FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}
FUNCTION {fin.entry}
{ duplicate$ empty$
    'pop$
    'write$
  if$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}
FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
        'skip$
        { after.sentence 'output.state := }
      if$
    }
  if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}


FUNCTION {add.colon}
{ duplicate$ empty$
    'skip$
    { ":" * add.blank }
  if$
}

FUNCTION {date.block}
{
  new.block
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}
FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}
FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}
STRINGS {z}
FUNCTION {remove.dots}
{ 'z :=
  ""
  { z empty$ not }
  { z #1 #1 substring$
    z #2 global.max$ substring$ 'z :=
    duplicate$ "." = 'pop$
      { * }
    if$
  }
  while$
}
FUNCTION {new.block.checka}
{ empty$
    'skip$
    'new.block
  if$
}
FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}
FUNCTION {new.sentence.checka}
{ empty$
    'skip$
    'new.sentence
  if$
}
FUNCTION {new.sentence.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.sentence
  if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}
FUNCTION {emphasize}
{ skip$ }

FUNCTION {embolden}
{ duplicate$ empty$
{ pop$ "" }
{ "\textbf{" swap$ * "}" * }
if$
}
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #5 <
    { "~" }
    { " " }
  if$
  swap$
}
FUNCTION {titto.space.prefix} %  always introduce a space
{ duplicate$ text.length$ #3 <
    { " " }
    { " " }
  if$
  swap$
}


FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
 % Here are the language-specific definitions for explicit words.
 % Each function has a name bbl.xxx where xxx is the English word.
 % The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "eds." }

FUNCTION {bbl.editor}
{ "ed." }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "edn." }

FUNCTION {bbl.volume}
{ "vol." }

FUNCTION {titto.bbl.volume} % for handling journals
{ "" }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "no." }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "pp." }

FUNCTION {bbl.page}
{ "p." }

FUNCTION {titto.bbl.pages} % for journals
{ "" }

FUNCTION {titto.bbl.page}  % for journals
{ "" }

FUNCTION {bbl.chapter}
{ "chap." }

FUNCTION {bbl.techrep}
{ "Tech. Rep." }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "Ph.D. thesis" }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"Jun."}

MACRO {jul} {"Jul."}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sep."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

MACRO {acmcs} {"ACM Comput. Surv."}

MACRO {acta} {"Acta Inf."}

MACRO {cacm} {"Commun. ACM"}

MACRO {ibmjrd} {"IBM J. Res. Dev."}

MACRO {ibmsj} {"IBM Syst.~J."}

MACRO {ieeese} {"IEEE Trans. Software Eng."}

MACRO {ieeetc} {"IEEE Trans. Comput."}

MACRO {ieeetcad}
 {"IEEE Trans. Comput. Aid. Des."}

MACRO {ipl} {"Inf. Process. Lett."}

MACRO {jacm} {"J.~ACM"}

MACRO {jcss} {"J.~Comput. Syst. Sci."}

MACRO {scp} {"Sci. Comput. Program."}

MACRO {sicomp} {"SIAM J. Comput."}

MACRO {tocs} {"ACM Trans. Comput. Syst."}

MACRO {tods} {"ACM Trans. Database Syst."}

MACRO {tog} {"ACM Trans. Graphic."}

MACRO {toms} {"ACM Trans. Math. Software"}

MACRO {toois} {"ACM Trans. Office Inf. Syst."}

MACRO {toplas} {"ACM Trans. Progr. Lang. Syst."}

MACRO {tcs} {"Theor. Comput. Sci."}

FUNCTION {bibinfo.check}
{ swap$
  duplicate$ missing$
    {
      pop$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ pop$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
FUNCTION {bibinfo.warn}
{ swap$
  duplicate$ missing$
    {
      swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ "empty " swap$ * " in " * cite$ * warning$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
FUNCTION {format.url}
{ url empty$
    { "" }
%    { "\urlprefix\url{" url * "}" * }
    { "\url{" url * "}" * }  % changed in titto-lncs-02.bst
  if$
}

FUNCTION {format.doi} % added in splncs04.bst
{ doi empty$
     { "" }
     { after.block 'output.state :=
       "\doi{" doi * "}" * }
  if$
}

INTEGERS { nameptr namesleft numnames }


STRINGS  { bibinfo}

FUNCTION {format.names}
{ 'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}{, jj}{, f{.}.}"
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              "," *
              t "others" =
                {
                  " " * bbl.etal *
                }
                { " " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.names.ed}
{
  'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{f{.}.~}{vv~}{ll}{ jj}"
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              "," *
              t "others" =
                {

                  " " * bbl.etal *
                }
                { " " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.authors}
{ author "author" format.names
}
FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
    {
      " " *
      get.bbl.editor
%      capitalize
   "(" swap$ * ")" *
      *
    }
  if$
}
FUNCTION {format.note}
{
 note empty$
    { "" }
    { note #1 #1 substring$
      duplicate$ "{" =
        'skip$
        { output.state mid.sentence =
          { "l" }
          { "u" }
        if$
        change.case$
        }
      if$
      note #2 global.max$ substring$ * "note" bibinfo.check
    }
  if$
}

FUNCTION {format.title}
{ title
  duplicate$ empty$ 'skip$
    { "t" change.case$ }
  if$
  "title" bibinfo.check
}
FUNCTION {output.bibitem}
{ newline$
  "\bibitem{" write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {n.dashify}
{
  't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

FUNCTION {word.in}
{ bbl.in capitalize
  ":" *
  " " * }

FUNCTION {format.date}
{
  month "month" bibinfo.check
  duplicate$ empty$
  year  "year"  bibinfo.check duplicate$ empty$
    { swap$ 'skip$
        { "there's a month but no year in " cite$ * warning$ }
      if$
      *
    }
    { swap$ 'skip$
        {
          swap$
          " " * swap$
        }
      if$
      *
      remove.dots
    }
  if$
  duplicate$ empty$
    'skip$
    {
      before.all 'output.state :=
    " (" swap$ * ")" *
    }
  if$
}
FUNCTION {format.btitle}
{ title "title" bibinfo.check
  duplicate$ empty$ 'skip$
    {
    }
  if$
}
FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}
FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { bbl.volume volume tie.or.space.prefix
      "volume" bibinfo.check * *
      series "series" bibinfo.check
      duplicate$ empty$ 'pop$
        { emphasize ", " * swap$ * }
      if$
      "volume and number" number either.or.check
    }
  if$
}
FUNCTION {format.number.series}
{ volume empty$
    { number empty$
        { series field.or.null }
        { output.state mid.sentence =
            { bbl.number }
            { bbl.number capitalize }
          if$
          number tie.or.space.prefix "number" bibinfo.check * *
          series empty$
            { "there's a number but no series in " cite$ * warning$ }
            { bbl.in space.word *
              series "series" bibinfo.check *
            }
          if$
        }
      if$
    }
    { "" }
  if$
}

FUNCTION {format.edition}
{ edition duplicate$ empty$ 'skip$
    {
      output.state mid.sentence =
        { "l" }
        { "t" }
      if$ change.case$
      "edition" bibinfo.check
      " " * bbl.edition *
    }
  if$
}
INTEGERS { multiresult }
FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
        { #1 'multiresult := }
        { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}
FUNCTION {format.pages}
{ pages duplicate$ empty$ 'skip$
    { duplicate$ multi.page.check
        {
          bbl.pages swap$
          n.dashify
        }
        {
          bbl.page swap$
        }
      if$
      tie.or.space.prefix
      "pages" bibinfo.check
      * *
    }
  if$
}
FUNCTION {format.journal.pages}
{ pages duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$
        { pop$ pop$ format.pages }
        {
          ", " *
          swap$
          n.dashify
          pages multi.page.check
            'titto.bbl.pages
            'titto.bbl.page
          if$
          swap$ tie.or.space.prefix
          "pages" bibinfo.check
          * *
          *
        }
      if$
    }
  if$
}
FUNCTION {format.journal.eid}
{ eid "eid" bibinfo.check
  duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$ 'skip$
      {
          ", " *
      }
      if$
      swap$ *
    }
  if$
}
FUNCTION {format.vol.num.pages} % this function is used only for journal entries
{ volume field.or.null embolden
  duplicate$ empty$ 'skip$
    {
%    bbl.volume swap$ tie.or.space.prefix
     titto.bbl.volume swap$ titto.space.prefix
%            rationale for the change above: for journals you don't want "vol." label
%            hence it does not make sense to attach the journal number to the label when
%            it is short
      "volume" bibinfo.check
      * *
      }
  if$
  number "number" bibinfo.check duplicate$ empty$ 'skip$
    {
      swap$ duplicate$ empty$
        { "there's a number but no volume in " cite$ * warning$ }
        'skip$
      if$
      swap$
      "(" swap$ * ")" *
    }
  if$ *
  eid empty$
    { format.journal.pages }
    { format.journal.eid }
  if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
        { bbl.chapter }
        { type "l" change.case$
          "type" bibinfo.check
        }
      if$
      chapter tie.or.space.prefix
      "chapter" bibinfo.check
      * *
      pages empty$
        'skip$
        { ", " * format.pages * }
      if$
    }
  if$
}

FUNCTION {format.booktitle}
{
  booktitle "booktitle" bibinfo.check
}
FUNCTION {format.in.ed.booktitle}
{ format.booktitle duplicate$ empty$ 'skip$
    {
%     editor "editor" format.names.ed duplicate$ empty$ 'pop$ % changed by titto
      editor "editor" format.names duplicate$ empty$ 'pop$
        {
          " " *
          get.bbl.editor
%          capitalize
          "(" swap$ * ") " *
          * swap$
          * }
      if$
      word.in swap$ *
    }
  if$
}
FUNCTION {empty.misc.check}
{ author empty$ title empty$ howpublished empty$
  month empty$ year empty$ note empty$
  and and and and and
  key empty$ not and
    { "all relevant fields are empty in " cite$ * warning$ }
    'skip$
  if$
}
FUNCTION {format.thesis.type}
{ type duplicate$ empty$
    'pop$
    { swap$ pop$
      "t" change.case$ "type" bibinfo.check
    }
  if$
}
FUNCTION {format.tr.number}
{ number "number" bibinfo.check
  type duplicate$ empty$
    { pop$ bbl.techrep }
    'skip$
  if$
  "type" bibinfo.check
  swap$ duplicate$ empty$
    { pop$ "t" change.case$ }
    { tie.or.space.prefix * * }
  if$
}
FUNCTION {format.article.crossref}
{
  key duplicate$ empty$
    { pop$
      journal duplicate$ empty$
        { "need key or journal for " cite$ * " to crossref " * crossref * warning$ }
        { "journal" bibinfo.check emphasize word.in swap$ * }
      if$
    }
    { word.in swap$ * " " *}
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.crossref.editor}
{ editor #1 "{vv~}{ll}" format.name$
  "editor" bibinfo.check
  editor num.names$ duplicate$
  #2 >
    { pop$
      "editor" bibinfo.check
      " " * bbl.etal
      *
    }
    { #2 <
        'skip$
        { editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            {
              "editor" bibinfo.check
              " " * bbl.etal
              *
            }
            {
             bbl.and space.word
              * editor #2 "{vv~}{ll}" format.name$
              "editor" bibinfo.check
              *
            }
          if$
        }
      if$
    }
  if$
}
FUNCTION {format.book.crossref}
{ volume duplicate$ empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      pop$ word.in
    }
    { bbl.volume
      capitalize
      swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
    }
  if$
  editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
        { series empty$
            { "need editor, key, or series for " cite$ * " to crossref " *
              crossref * warning$
              "" *
            }
            { series emphasize * }
          if$
        }
        { key * }
      if$
    }
    { format.crossref.editor * }
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.incoll.inproc.crossref}
{
  editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
        { format.booktitle duplicate$ empty$
            { "need editor, key, or booktitle for " cite$ * " to crossref " *
              crossref * warning$
            }
            { word.in swap$ * }
          if$
        }
        { word.in key * " " *}
      if$
    }
    { word.in format.crossref.editor * " " *}
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.org.or.pub}
{ 't :=
  ""
  address empty$ t empty$ and
    'skip$
    {
      t empty$
        { address "address" bibinfo.check *
        }
        { t *
          address empty$
            'skip$
            { ", " * address "address" bibinfo.check * }
          if$
        }
      if$
    }
  if$
}
FUNCTION {format.publisher.address}
{ publisher "publisher" bibinfo.warn format.org.or.pub
}

FUNCTION {format.organization.address}
{ organization "organization" bibinfo.check format.org.or.pub
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    {
      journal
      "journal" bibinfo.check
      "journal" output.check
      add.blank
      format.vol.num.pages output
      format.date "year" output.check
    }
    { format.article.crossref output.nonnull
      format.pages output
    }
  if$
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}
FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      add.colon
    }
    { format.authors output.nonnull
      add.colon
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      new.block
      new.sentence
      format.number.series output
      format.publisher.address output
    }
    {
      new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}
FUNCTION {booklet}
{ output.bibitem
  format.authors output
  add.colon
  new.block
  format.title "title" output.check
  new.block
  howpublished "howpublished" bibinfo.check output
  address "address" bibinfo.check output
  format.date output
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      add.colon
    }
    { format.authors output.nonnull
      add.colon
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    {
      format.bvolume output
      format.chapter.pages "chapter and pages" output.check
      new.block
      new.sentence
      format.number.series output
      format.publisher.address output
    }
    {
      format.chapter.pages "chapter and pages" output.check
      new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.chapter.pages output
      new.sentence
      format.number.series output
      format.publisher.address output
      format.edition output
      format.date "year" output.check
    }
    { format.incoll.inproc.crossref output.nonnull
      format.chapter.pages output
    }
  if$
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}
FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      new.sentence % added by titto
      format.bvolume output
      format.pages output
      new.sentence
      format.number.series output
      publisher empty$
        { format.organization.address output }
        { organization "organization" bibinfo.check output
          format.publisher.address output
        }
      if$
      format.date "year" output.check
    }
    { format.incoll.inproc.crossref output.nonnull
      format.pages output
    }
  if$
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}
FUNCTION {conference} { inproceedings }
FUNCTION {manual}
{ output.bibitem
  author empty$
    { organization "organization" bibinfo.check
      duplicate$ empty$ 'pop$
        { output
          address "address" bibinfo.check output
        }
      if$
    }
    { format.authors output.nonnull }
  if$
  add.colon
  new.block
  format.btitle "title" output.check
  author empty$
    { organization empty$
        {
          address new.block.checka
          address "address" bibinfo.check output
        }
        'skip$
      if$
    }
    {
      organization address new.block.checkb
      organization "organization" bibinfo.check output
      address "address" bibinfo.check output
    }
  if$
  format.edition output
  format.date output
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.btitle
  "title" output.check
  new.block
  bbl.mthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {misc}
{ output.bibitem
  format.authors output
  add.colon
  title howpublished new.block.checkb
  format.title output
  howpublished new.block.checka
  howpublished "howpublished" bibinfo.check output
  format.date output
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
  empty.misc.check
}
FUNCTION {phdthesis}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.btitle
  "title" output.check
  new.block
  bbl.phdthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
  editor empty$
    { organization "organization" bibinfo.check output
    }
    { format.editors output.nonnull }
  if$
  add.colon
  new.block
  format.btitle "title" output.check
  format.bvolume output
  editor empty$
    { publisher empty$
        {  format.number.series output }
        {
          new.sentence
          format.number.series output
          format.publisher.address output
        }
      if$
    }
    { publisher empty$
        {
          new.sentence
          format.number.series output
          format.organization.address output }
        {
          new.sentence
          format.number.series output
          organization "organization" bibinfo.check output
          format.publisher.address output
        }
      if$
     }
  if$
      format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title
  "title" output.check
  new.block
  format.tr.number output.nonnull
  institution "institution" bibinfo.warn output
  address "address" bibinfo.check output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title "title" output.check
  format.date output
%  new.block
  format.url output
%  new.block
  format.note "note" output.check
  fin.entry
}

FUNCTION {default.type} { misc }
READ
FUNCTION {sortify}
{ purify$
  "l" change.case$
}
INTEGERS { len }
FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}
FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{ll{ }}{  ff{ }}{  jj{ }}"
      format.name$ 't :=
      nameptr #1 >
        {
          "   "  *
          namesleft #1 = t "others" = and
            { "zzzzz" * }
            { t sortify * }
          if$
        }
        { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}
FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {author.organization.sort}
{ author empty$
    { organization empty$
        { key empty$
            { "to sort, need author, organization, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { "The " #4 organization chop.word sortify }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {editor.organization.sort}
{ editor empty$
    { organization empty$
        { key empty$
            { "to sort, need editor, organization, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { "The " #4 organization chop.word sortify }
      if$
    }
    { editor sort.format.names }
  if$
}
FUNCTION {presort}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.organization.sort
        { type$ "manual" =
            'author.organization.sort
            'author.sort
          if$
        }
      if$
    }
  if$
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}
ITERATE {presort}
SORT
STRINGS { longest.label }
INTEGERS { number.label longest.label.width }
FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
  #1 'number.label :=
  #0 'longest.label.width :=
}
FUNCTION {longest.label.pass}
{ number.label int.to.str$ 'label :=
  number.label #1 + 'number.label :=
  label width$ longest.label.width >
    { label 'longest.label :=
      label width$ 'longest.label.width :=
    }
    'skip$
  if$
}
EXECUTE {initialize.longest.label}
ITERATE {longest.label.pass}
FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{"  longest.label  * "}" *
  write$ newline$
  "\providecommand{\url}[1]{\texttt{#1}}"
  write$ newline$
  "\providecommand{\urlprefix}{URL }"
  write$ newline$
  "\providecommand{\doi}[1]{https://doi.org/#1}"
  write$ newline$
}
EXECUTE {begin.bib}
EXECUTE {init.state.consts}
ITERATE {call.type$}
FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}
EXECUTE {end.bib}
%% End of customized bst file
%%
%% End of file `titto.bst'.


==> sections/inductive_transfer_learning/selection_and_ensembles/figures/blended_learning.tex <==
\resizebox{0.95\textwidth}{!}{%
    \begin{tikzpicture}

        \draw[thick,->] (0,0) -- (10.5,0) node[anchor=north, xshift=-8.5cm, yshift=-0.1cm] {available training data};
        \draw[thick,->] (0,0) -- (0,5.5) node[anchor=south west, yshift=-3.75cm, xshift=-0.1cm, rotate=90] {weighting};

        %\draw[step=1cm,gray,very thin] (0, 0) grid (10, 5);

        \draw[color=black,dashed, thick] (0,0) .. controls (10,0) and (3,4.5) .. (10,4.9) node[anchor=south, xshift=-1cm] {target model};
        \draw[color=black,dotted, thick] (0,0) .. controls (2.5,0) and (2.5,5) .. (5,5) node[anchor=south] {'Blended Transfer'};
        \draw[color=black,dotted, thick] (5,5) .. controls (7.5, 5) and (7.5, 0) .. (10,0.1);
        \draw[color=black, dash dot, thick] (0,5) .. controls (5, 5) and (0,0) .. (10, 0) node[anchor=south, xshift=-8.5cm, yshift=5cm] {source models};


    \end{tikzpicture}
}

==> splncs <==
%% BibTeX bibliography style `splncs03'
%%
%% BibTeX bibliography style for use with numbered references in
%% Springer Verlag's "Lecture Notes in Computer Science" series.
%% (See Springer's documentation for llncs.cls for
%% more details of the suggested reference format.)  Note that this
%% file will not work for author-year style citations.
%%
%% Use \documentclass{llncs} and \bibliographystyle{splncs03}, and cite
%% a reference with (e.g.) \cite{smith77} to get a "[1]" in the text.
%%
%% This file comes to you courtesy of Maurizio "Titto" Patrignani of
%% Dipartimento di Informatica e Automazione Universita' Roma Tre
%%
%% ================================================================================================
%% This was file `titto-lncs-02.bst' produced on Wed Apr 1, 2009
%% Edited by hand by titto based on `titto-lncs-01.bst' (see below)
%%
%% CHANGES (with respect to titto-lncs-01.bst):
%% - Removed the call to \urlprefix (thus no "URL" string is added to the output)
%% ================================================================================================
%% This was file `titto-lncs-01.bst' produced on Fri Aug 22, 2008
%% Edited by hand by titto based on `titto.bst' (see below)
%%
%% CHANGES (with respect to titto.bst):
%% - Removed the "capitalize" command for editors string "(eds.)" and "(ed.)"
%% - Introduced the functions titto.bbl.pages and titto.bbl.page for journal pages (without "pp.")
%% - Added a new.sentence command to separate with a dot booktitle and series in the inproceedings
%% - Commented all new.block commands before urls and notes (to separate them with a comma)
%% - Introduced the functions titto.bbl.volume for handling journal volumes (without "vol." label)
%% - Used for editors the same name conventions used for authors (see function format.in.ed.booktitle)
%% - Removed a \newblock to avoid long spaces between title and "In: ..."
%% - Added function titto.space.prefix to add a space instead of "~" after the (removed) "vol." label
%% - Added doi
%% ================================================================================================
%% This was file `titto.bst',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `vonx,nm-rvvc,yr-par,jttl-rm,volp-com,jwdpg,jwdvol,numser,ser-vol,jnm-x,btit-rm,bt-rm,edparxc,bkedcap,au-col,in-col,fin-bare,pp,ed,abr,mth-bare,xedn,jabr,and-com,and-com-ed,xand,url,url-blk,em-x,nfss,')
%% ----------------------------------------
%% *** Tentative .bst file for Springer LNCS ***
%%
%% Copyright 1994-2007 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2007/04/24 4.20 (PWD, AO, DPC)]
 %   For use with BibTeX version 0.99a or later
 %-------------------------------------------------------------------
 % This bibliography style file is intended for texts in ENGLISH
 % This is a numerical citation style, and as such is standard LaTeX.
 % It requires no extra package to interface to the main text.
 % The form of the \bibitem entries is
 %   \bibitem{key}...
 % Usage of \cite is as follows:
 %   \cite{key} ==>>          [#]
 %   \cite[chap. 2]{key} ==>> [#, chap. 2]
 % where # is a number determined by the ordering in the reference list.
 % The order in the reference list is alphabetical by authors.
 %---------------------------------------------------------------------

ENTRY
  { address
    author
    booktitle
    chapter
    doi
    edition
    editor
    eid
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    url
    volume
    year
  }
  {}
  { label }
INTEGERS { output.state before.all mid.sentence after.sentence after.block }
FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}
STRINGS { s t}
FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
        { add.period$ write$
%          newline$
%          "\newblock " write$  % removed for titto-lncs-01
          " " write$            % to avoid long spaces between title and "In: ..."
        }
        { output.state before.all =
            'write$
            { add.period$ " " * write$ }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}
FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}
FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}
FUNCTION {fin.entry}
{ duplicate$ empty$
    'pop$
    'write$
  if$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}
FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
        'skip$
        { after.sentence 'output.state := }
      if$
    }
  if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}


FUNCTION {add.colon}
{ duplicate$ empty$
    'skip$
    { ":" * add.blank }
  if$
}

FUNCTION {date.block}
{
  new.block
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}
FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}
FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}
STRINGS {z}
FUNCTION {remove.dots}
{ 'z :=
  ""
  { z empty$ not }
  { z #1 #1 substring$
    z #2 global.max$ substring$ 'z :=
    duplicate$ "." = 'pop$
      { * }
    if$
  }
  while$
}
FUNCTION {new.block.checka}
{ empty$
    'skip$
    'new.block
  if$
}
FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}
FUNCTION {new.sentence.checka}
{ empty$
    'skip$
    'new.sentence
  if$
}
FUNCTION {new.sentence.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.sentence
  if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}
FUNCTION {emphasize}
{ skip$ }

FUNCTION {embolden}
{ duplicate$ empty$
{ pop$ "" }
{ "\textbf{" swap$ * "}" * }
if$
}
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #5 <
    { "~" }
    { " " }
  if$
  swap$
}
FUNCTION {titto.space.prefix} %  always introduce a space
{ duplicate$ text.length$ #3 <
    { " " }
    { " " }
  if$
  swap$
}


FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
 % Here are the language-specific definitions for explicit words.
 % Each function has a name bbl.xxx where xxx is the English word.
 % The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "eds." }

FUNCTION {bbl.editor}
{ "ed." }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "edn." }

FUNCTION {bbl.volume}
{ "vol." }

FUNCTION {titto.bbl.volume} % for handling journals
{ "" }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "no." }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "pp." }

FUNCTION {bbl.page}
{ "p." }

FUNCTION {titto.bbl.pages} % for journals
{ "" }

FUNCTION {titto.bbl.page}  % for journals
{ "" }

FUNCTION {bbl.chapter}
{ "chap." }

FUNCTION {bbl.techrep}
{ "Tech. Rep." }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "Ph.D. thesis" }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"Jun."}

MACRO {jul} {"Jul."}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sep."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

MACRO {acmcs} {"ACM Comput. Surv."}

MACRO {acta} {"Acta Inf."}

MACRO {cacm} {"Commun. ACM"}

MACRO {ibmjrd} {"IBM J. Res. Dev."}

MACRO {ibmsj} {"IBM Syst.~J."}

MACRO {ieeese} {"IEEE Trans. Software Eng."}

MACRO {ieeetc} {"IEEE Trans. Comput."}

MACRO {ieeetcad}
 {"IEEE Trans. Comput. Aid. Des."}

MACRO {ipl} {"Inf. Process. Lett."}

MACRO {jacm} {"J.~ACM"}

MACRO {jcss} {"J.~Comput. Syst. Sci."}

MACRO {scp} {"Sci. Comput. Program."}

MACRO {sicomp} {"SIAM J. Comput."}

MACRO {tocs} {"ACM Trans. Comput. Syst."}

MACRO {tods} {"ACM Trans. Database Syst."}

MACRO {tog} {"ACM Trans. Graphic."}

MACRO {toms} {"ACM Trans. Math. Software"}

MACRO {toois} {"ACM Trans. Office Inf. Syst."}

MACRO {toplas} {"ACM Trans. Progr. Lang. Syst."}

MACRO {tcs} {"Theor. Comput. Sci."}

FUNCTION {bibinfo.check}
{ swap$
  duplicate$ missing$
    {
      pop$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ pop$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
FUNCTION {bibinfo.warn}
{ swap$
  duplicate$ missing$
    {
      swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ "empty " swap$ * " in " * cite$ * warning$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
FUNCTION {format.url}
{ url empty$
    { "" }
%    { "\urlprefix\url{" url * "}" * }
    { "\url{" url * "}" * }  % changed in titto-lncs-02.bst
  if$
}

FUNCTION {format.doi} % added in splncs04.bst
{ doi empty$
     { "" }
     { after.block 'output.state :=
       "\doi{" doi * "}" * }
  if$
}

INTEGERS { nameptr namesleft numnames }


STRINGS  { bibinfo}

FUNCTION {format.names}
{ 'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}{, jj}{, f{.}.}"
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              "," *
              t "others" =
                {
                  " " * bbl.etal *
                }
                { " " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.names.ed}
{
  'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{f{.}.~}{vv~}{ll}{ jj}"
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              "," *
              t "others" =
                {

                  " " * bbl.etal *
                }
                { " " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.authors}
{ author "author" format.names
}
FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
    {
      " " *
      get.bbl.editor
%      capitalize
   "(" swap$ * ")" *
      *
    }
  if$
}
FUNCTION {format.note}
{
 note empty$
    { "" }
    { note #1 #1 substring$
      duplicate$ "{" =
        'skip$
        { output.state mid.sentence =
          { "l" }
          { "u" }
        if$
        change.case$
        }
      if$
      note #2 global.max$ substring$ * "note" bibinfo.check
    }
  if$
}

FUNCTION {format.title}
{ title
  duplicate$ empty$ 'skip$
    { "t" change.case$ }
  if$
  "title" bibinfo.check
}
FUNCTION {output.bibitem}
{ newline$
  "\bibitem{" write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {n.dashify}
{
  't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

FUNCTION {word.in}
{ bbl.in capitalize
  ":" *
  " " * }

FUNCTION {format.date}
{
  month "month" bibinfo.check
  duplicate$ empty$
  year  "year"  bibinfo.check duplicate$ empty$
    { swap$ 'skip$
        { "there's a month but no year in " cite$ * warning$ }
      if$
      *
    }
    { swap$ 'skip$
        {
          swap$
          " " * swap$
        }
      if$
      *
      remove.dots
    }
  if$
  duplicate$ empty$
    'skip$
    {
      before.all 'output.state :=
    " (" swap$ * ")" *
    }
  if$
}
FUNCTION {format.btitle}
{ title "title" bibinfo.check
  duplicate$ empty$ 'skip$
    {
    }
  if$
}
FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}
FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { bbl.volume volume tie.or.space.prefix
      "volume" bibinfo.check * *
      series "series" bibinfo.check
      duplicate$ empty$ 'pop$
        { emphasize ", " * swap$ * }
      if$
      "volume and number" number either.or.check
    }
  if$
}
FUNCTION {format.number.series}
{ volume empty$
    { number empty$
        { series field.or.null }
        { output.state mid.sentence =
            { bbl.number }
            { bbl.number capitalize }
          if$
          number tie.or.space.prefix "number" bibinfo.check * *
          series empty$
            { "there's a number but no series in " cite$ * warning$ }
            { bbl.in space.word *
              series "series" bibinfo.check *
            }
          if$
        }
      if$
    }
    { "" }
  if$
}

FUNCTION {format.edition}
{ edition duplicate$ empty$ 'skip$
    {
      output.state mid.sentence =
        { "l" }
        { "t" }
      if$ change.case$
      "edition" bibinfo.check
      " " * bbl.edition *
    }
  if$
}
INTEGERS { multiresult }
FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
        { #1 'multiresult := }
        { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}
FUNCTION {format.pages}
{ pages duplicate$ empty$ 'skip$
    { duplicate$ multi.page.check
        {
          bbl.pages swap$
          n.dashify
        }
        {
          bbl.page swap$
        }
      if$
      tie.or.space.prefix
      "pages" bibinfo.check
      * *
    }
  if$
}
FUNCTION {format.journal.pages}
{ pages duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$
        { pop$ pop$ format.pages }
        {
          ", " *
          swap$
          n.dashify
          pages multi.page.check
            'titto.bbl.pages
            'titto.bbl.page
          if$
          swap$ tie.or.space.prefix
          "pages" bibinfo.check
          * *
          *
        }
      if$
    }
  if$
}
FUNCTION {format.journal.eid}
{ eid "eid" bibinfo.check
  duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$ 'skip$
      {
          ", " *
      }
      if$
      swap$ *
    }
  if$
}
FUNCTION {format.vol.num.pages} % this function is used only for journal entries
{ volume field.or.null embolden
  duplicate$ empty$ 'skip$
    {
%    bbl.volume swap$ tie.or.space.prefix
     titto.bbl.volume swap$ titto.space.prefix
%            rationale for the change above: for journals you don't want "vol." label
%            hence it does not make sense to attach the journal number to the label when
%            it is short
      "volume" bibinfo.check
      * *
      }
  if$
  number "number" bibinfo.check duplicate$ empty$ 'skip$
    {
      swap$ duplicate$ empty$
        { "there's a number but no volume in " cite$ * warning$ }
        'skip$
      if$
      swap$
      "(" swap$ * ")" *
    }
  if$ *
  eid empty$
    { format.journal.pages }
    { format.journal.eid }
  if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
        { bbl.chapter }
        { type "l" change.case$
          "type" bibinfo.check
        }
      if$
      chapter tie.or.space.prefix
      "chapter" bibinfo.check
      * *
      pages empty$
        'skip$
        { ", " * format.pages * }
      if$
    }
  if$
}

FUNCTION {format.booktitle}
{
  booktitle "booktitle" bibinfo.check
}
FUNCTION {format.in.ed.booktitle}
{ format.booktitle duplicate$ empty$ 'skip$
    {
%     editor "editor" format.names.ed duplicate$ empty$ 'pop$ % changed by titto
      editor "editor" format.names duplicate$ empty$ 'pop$
        {
          " " *
          get.bbl.editor
%          capitalize
          "(" swap$ * ") " *
          * swap$
          * }
      if$
      word.in swap$ *
    }
  if$
}
FUNCTION {empty.misc.check}
{ author empty$ title empty$ howpublished empty$
  month empty$ year empty$ note empty$
  and and and and and
  key empty$ not and
    { "all relevant fields are empty in " cite$ * warning$ }
    'skip$
  if$
}
FUNCTION {format.thesis.type}
{ type duplicate$ empty$
    'pop$
    { swap$ pop$
      "t" change.case$ "type" bibinfo.check
    }
  if$
}
FUNCTION {format.tr.number}
{ number "number" bibinfo.check
  type duplicate$ empty$
    { pop$ bbl.techrep }
    'skip$
  if$
  "type" bibinfo.check
  swap$ duplicate$ empty$
    { pop$ "t" change.case$ }
    { tie.or.space.prefix * * }
  if$
}
FUNCTION {format.article.crossref}
{
  key duplicate$ empty$
    { pop$
      journal duplicate$ empty$
        { "need key or journal for " cite$ * " to crossref " * crossref * warning$ }
        { "journal" bibinfo.check emphasize word.in swap$ * }
      if$
    }
    { word.in swap$ * " " *}
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.crossref.editor}
{ editor #1 "{vv~}{ll}" format.name$
  "editor" bibinfo.check
  editor num.names$ duplicate$
  #2 >
    { pop$
      "editor" bibinfo.check
      " " * bbl.etal
      *
    }
    { #2 <
        'skip$
        { editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            {
              "editor" bibinfo.check
              " " * bbl.etal
              *
            }
            {
             bbl.and space.word
              * editor #2 "{vv~}{ll}" format.name$
              "editor" bibinfo.check
              *
            }
          if$
        }
      if$
    }
  if$
}
FUNCTION {format.book.crossref}
{ volume duplicate$ empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      pop$ word.in
    }
    { bbl.volume
      capitalize
      swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
    }
  if$
  editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
        { series empty$
            { "need editor, key, or series for " cite$ * " to crossref " *
              crossref * warning$
              "" *
            }
            { series emphasize * }
          if$
        }
        { key * }
      if$
    }
    { format.crossref.editor * }
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.incoll.inproc.crossref}
{
  editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
        { format.booktitle duplicate$ empty$
            { "need editor, key, or booktitle for " cite$ * " to crossref " *
              crossref * warning$
            }
            { word.in swap$ * }
          if$
        }
        { word.in key * " " *}
      if$
    }
    { word.in format.crossref.editor * " " *}
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.org.or.pub}
{ 't :=
  ""
  address empty$ t empty$ and
    'skip$
    {
      t empty$
        { address "address" bibinfo.check *
        }
        { t *
          address empty$
            'skip$
            { ", " * address "address" bibinfo.check * }
          if$
        }
      if$
    }
  if$
}
FUNCTION {format.publisher.address}
{ publisher "publisher" bibinfo.warn format.org.or.pub
}

FUNCTION {format.organization.address}
{ organization "organization" bibinfo.check format.org.or.pub
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    {
      journal
      "journal" bibinfo.check
      "journal" output.check
      add.blank
      format.vol.num.pages output
      format.date "year" output.check
    }
    { format.article.crossref output.nonnull
      format.pages output
    }
  if$
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}
FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      add.colon
    }
    { format.authors output.nonnull
      add.colon
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      new.block
      new.sentence
      format.number.series output
      format.publisher.address output
    }
    {
      new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}
FUNCTION {booklet}
{ output.bibitem
  format.authors output
  add.colon
  new.block
  format.title "title" output.check
  new.block
  howpublished "howpublished" bibinfo.check output
  address "address" bibinfo.check output
  format.date output
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      add.colon
    }
    { format.authors output.nonnull
      add.colon
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    {
      format.bvolume output
      format.chapter.pages "chapter and pages" output.check
      new.block
      new.sentence
      format.number.series output
      format.publisher.address output
    }
    {
      format.chapter.pages "chapter and pages" output.check
      new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.chapter.pages output
      new.sentence
      format.number.series output
      format.publisher.address output
      format.edition output
      format.date "year" output.check
    }
    { format.incoll.inproc.crossref output.nonnull
      format.chapter.pages output
    }
  if$
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}
FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      new.sentence % added by titto
      format.bvolume output
      format.pages output
      new.sentence
      format.number.series output
      publisher empty$
        { format.organization.address output }
        { organization "organization" bibinfo.check output
          format.publisher.address output
        }
      if$
      format.date "year" output.check
    }
    { format.incoll.inproc.crossref output.nonnull
      format.pages output
    }
  if$
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}
FUNCTION {conference} { inproceedings }
FUNCTION {manual}
{ output.bibitem
  author empty$
    { organization "organization" bibinfo.check
      duplicate$ empty$ 'pop$
        { output
          address "address" bibinfo.check output
        }
      if$
    }
    { format.authors output.nonnull }
  if$
  add.colon
  new.block
  format.btitle "title" output.check
  author empty$
    { organization empty$
        {
          address new.block.checka
          address "address" bibinfo.check output
        }
        'skip$
      if$
    }
    {
      organization address new.block.checkb
      organization "organization" bibinfo.check output
      address "address" bibinfo.check output
    }
  if$
  format.edition output
  format.date output
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.btitle
  "title" output.check
  new.block
  bbl.mthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {misc}
{ output.bibitem
  format.authors output
  add.colon
  title howpublished new.block.checkb
  format.title output
  howpublished new.block.checka
  howpublished "howpublished" bibinfo.check output
  format.date output
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
  empty.misc.check
}
FUNCTION {phdthesis}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.btitle
  "title" output.check
  new.block
  bbl.phdthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
  editor empty$
    { organization "organization" bibinfo.check output
    }
    { format.editors output.nonnull }
  if$
  add.colon
  new.block
  format.btitle "title" output.check
  format.bvolume output
  editor empty$
    { publisher empty$
        {  format.number.series output }
        {
          new.sentence
          format.number.series output
          format.publisher.address output
        }
      if$
    }
    { publisher empty$
        {
          new.sentence
          format.number.series output
          format.organization.address output }
        {
          new.sentence
          format.number.series output
          organization "organization" bibinfo.check output
          format.publisher.address output
        }
      if$
     }
  if$
      format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title
  "title" output.check
  new.block
  format.tr.number output.nonnull
  institution "institution" bibinfo.warn output
  address "address" bibinfo.check output
  format.date "year" output.check
%  new.block
  format.doi output
  format.url output
%  new.block
  format.note output
  fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
  format.authors "author" output.check
  add.colon
  new.block
  format.title "title" output.check
  format.date output
%  new.block
  format.url output
%  new.block
  format.note "note" output.check
  fin.entry
}

FUNCTION {default.type} { misc }
READ
FUNCTION {sortify}
{ purify$
  "l" change.case$
}
INTEGERS { len }
FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}
FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{ll{ }}{  ff{ }}{  jj{ }}"
      format.name$ 't :=
      nameptr #1 >
        {
          "   "  *
          namesleft #1 = t "others" = and
            { "zzzzz" * }
            { t sortify * }
          if$
        }
        { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}
FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {author.organization.sort}
{ author empty$
    { organization empty$
        { key empty$
            { "to sort, need author, organization, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { "The " #4 organization chop.word sortify }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {editor.organization.sort}
{ editor empty$
    { organization empty$
        { key empty$
            { "to sort, need editor, organization, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { "The " #4 organization chop.word sortify }
      if$
    }
    { editor sort.format.names }
  if$
}
FUNCTION {presort}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.organization.sort
        { type$ "manual" =
            'author.organization.sort
            'author.sort
          if$
        }
      if$
    }
  if$
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}
ITERATE {presort}
SORT
STRINGS { longest.label }
INTEGERS { number.label longest.label.width }
FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
  #1 'number.label :=
  #0 'longest.label.width :=
}
FUNCTION {longest.label.pass}
{ number.label int.to.str$ 'label :=
  number.label #1 + 'number.label :=
  label width$ longest.label.width >
    { label 'longest.label :=
      label width$ 'longest.label.width :=
    }
    'skip$
  if$
}
EXECUTE {initialize.longest.label}
ITERATE {longest.label.pass}
FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{"  longest.label  * "}" *
  write$ newline$
  "\providecommand{\url}[1]{\texttt{#1}}"
  write$ newline$
  "\providecommand{\urlprefix}{URL }"
  write$ newline$
  "\providecommand{\doi}[1]{https://doi.org/#1}"
  write$ newline$
}
EXECUTE {begin.bib}
EXECUTE {init.state.consts}
ITERATE {call.type$}
FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}
EXECUTE {end.bib}
%% End of customized bst file
%%
%% End of file `titto.bst'.

